Algorithms and Statistical Models for Scientific Discovery in the Petabyte Era

The field of astronomy has arrived at a turning point in terms of size and complexity of both datasets and scientific collaboration. Commensurately, algorithms and statistical models have begun to adapt --- e.g., via the onset of artificial intelligence --- which itself presents new challenges and opportunities for growth. This white paper aims to offer guidance and ideas for how we can evolve our technical and collaborative frameworks to promote efficient algorithmic development and take advantage of opportunities for scientific discovery in the petabyte era. We discuss challenges for discovery in large and complex data sets; challenges and requirements for the next stage of development of statistical methodologies and algorithmic tool sets; how we might change our paradigms of collaboration and education; and the ethical implications of scientists' contributions to widely applicable algorithms and computational modeling. We start with six distinct recommendations that are supported by the commentary following them. This white paper is related to a larger corpus of effort that has taken place within and around the Petabytes to Science Workshops (https://petabytestoscience.github.io/).

==> abstract.tex <==

% \keywords{
% Astronomy, Astrophysics, Work Force, Software, Algorithms, High-performance Computing, High-throughput Computing, Networking, Machine Learning, Cloud computing, Education, Management, Outreach
% }

%\textbf{Thematic Areas:} \hspace*{20pt} $\boxtimes$ Activity \hspace*{20pt} $\square$ Project \hspace*{20pt} $\boxtimes$ State of the Profession 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{abstract}
The field of astronomy has arrived at a turning point in terms of size and complexity of both datasets and scientific collaboration. 
Commensurately, algorithms and statistical models have begun to adapt --- e.g., via the onset of artificial intelligence --- which itself presents new challenges and opportunities for growth.
This white paper aims to offer guidance and ideas for how we can evolve our technical and collaborative frameworks to promote efficient algorithmic development and take advantage of opportunities for scientific discovery in the petabyte era.
We discuss challenges for discovery in large and complex data sets; challenges and requirements for the next stage of development of statistical methodologies and algorithmic tool sets; how we might change our paradigms of collaboration and education; and the ethical implications of scientists' contributions to widely applicable algorithms and computational modeling. 
We conclude with six distinct recommendations.

% \begin{enumerate}
%     \item More work is being performed in collaborations
%     \item Additionally the onset of new high-performance algorithms is disrupting this developing collaborative paradigm. 
%     \item Data sets are becoming larger and more multi-modal.
%     \item The current collaborative and educational frameworks continue to provide privileged access to computational tools and learning opportunities. 
%     \item But, we don't yet have a plan to develop new algorithms, collaborative structures, and educational frameworks that will allow us to take advantage of new data complexities or to change the disproportionate access to science and computational tools.
%     \item 
%     \item ethics implications
% \end{enumerate}

\end{abstract}



% At present, the process of hypothesis-generation in astronomy has two pathways. One is theoretical, wherein predictions from theory provide hypotheses that can be tested with observations. The other is observational, wherein surprising objects and patterns are found in data and later explored. As theory comes to depend on larger and larger simulations, and observational data sets grow to surpass the petabyte scale, both pathways are under threat. With such large data sets, the classical mode of visual, human exploration has become too slow and painstaking to find new objects and new correlations. But without new hypotheses in the 2020s, there will be no astronomy in the 2030s.

% We argue that the path forward is through the construction of intuitive, trustworthy, robust, and deployable algorithms for the exploration of large, high-dimensional data sets. Investigations show that purpose-built machine learning algorithms, coupled with deep sub-domain knowledge, can successfully pull out hitherto unknown objects, significantly advancing our understanding of our universe. Unfortunately, any successful exploration requires a) deep algorithmic and implementation knowledge, b) deep physical and observational domain knowledge, c) continued support and development, and d) luck. Deep algorithmic knowledge is necessary because off-the-shelf algorithms usually need significant adaptation to work with heteroscedastic and censored astronomical data. Deep observational domain knowledge is needed because outlier objects are often artifacts and surprising trends may be imprints of the data collection method. Deep physical domain knowledge is needed to make sense of the result, and understand its place in the cosmos and in the research ecosystem. Finally, not all searches will return results; a modicum of luck is needed. The confluence of these elements is rare, and technology for bringing them to bear on next-generation data sets has not yet been developed.

% We, therefore, propose that funding agencies fund the creation and maintenance of ``discovery engines'' --- tools that allow astronomers without deep algorithmic knowledge to explore the edges of data spaces, hunting for outliers and new trends. These engines should be hosted near the data when needed but should be initiated by the astronomical and methods communities.



% %%%%% collaboration


% The past decade has seen rapid change in the algorithmic, computational, and statistical landscape. We have seen the rise of new ``standard'' programming languages and libraries (e.g. python and astropy). There has been a proliferation of new algorithmic and statistical techniques ---  from improvements in image processing and compression to the rise of deep neural networks as a powerful suite of tools for machine learning. We have seen the rise of new computational modalities, such as cloud computing and “software as a service.” Even the basic mechanics of computation is undergoing a shift, with the availability of specialized hardware such as GPUs and TPUs, which require a new domain of knowledge to efficiently deploy solutions. Moreover, there is no reason to expect the pace of innovation to drop off anytime soon.

% The rapid pace of advancement means that it is no longer possible for a single astronomer or even a small team of astronomers to build the necessary depth of expertise in all of these areas. Yet these technologies may be critical to maximizing the scientific reach of new research. New technologies spring up quickly, and the astronomical community needs to balance the cost of learning the new technologies with the benefits they provide. It is not reasonable to expect every astronomer to keep up with all of the advances.

% In cases where collaborations exist today, there can be a variety of complicating challenges. There is currently no established marketplace for matching difficult problems in the astronomy domain to relevant experts outside an astronomer's network. The resulting in-depth collaborations have start-up overhead as the external experts learn enough about the problem domain to be helpful. Short-term engagements can suffer from a lack of depth or insufficiently productionized solutions. Even in longer-term engagements, there can be misalignment between the parties due to the different incentives. For example, statisticians and computer scientists in academia are primarily recognized for only the novel contributions to their own fields. Papers that apply existing methodologies to new problems are not considered significant contributions to their fields. Similarly, members of the astronomy community are not fully recognized for their algorithmic contributions.

% In education, we have started to make progress in providing a foundation in statistics and algorithms. However, it is not uniformly available across our community: there is significantly smaller access at smaller colleges and for communities that are traditionally underrepresented in astronomy, physics, and computing. The determination of what constitutes an appropriate curriculum will require a balance of priorities. We should provide the foundations of statistics/algorithmic design appropriate for the broader science community, as well as teach specialized skills (e.g., optimization, compilers) that may benefit a smaller, but crucial, set of researchers who will engage in the development and implementation of computing and software frameworks.

% We recommend that a new approach for interdisciplinary collaboration and education be adopted within astronomy. New modalities for the long-term engagement of algorithmic and statistical expertise outside of astronomy will need to be developed. Open educational resources that can be used in teaching statistics, and algorithms, and machine or computational learning will require coordinated and sustained efforts to integrate current resources within a broad curriculum and to make them easily accessible.




==> aglossary.tex <==
% DO NOT EDIT - generated by /Users/womullan/LSSTgit/lsst-texmf/bin/generateAcronyms.py from https://lsst-texmf.lsst.io/.
\newglossaryentry {1D} {name={1D}, description={One-dimensional}}
\newglossaryentry {2D} {name={2D}, description={Two-dimensional}}
\newglossaryentry {3D} {name={3D}, description={Three-dimensional}}
\newglossaryentry {AAG} {name={AAG}, description={Astronomy and Astrophysics Research Grants, an \gls{NSF} program}}
\newacronym {AAS} {AAS} {American Astronomical Society}
\newacronym {ADS} {ADS} {Astrophysics Data System}
\newglossaryentry {AI} {name={AI}, description={Artificial Intelligence, used to cover many machine learning algorithms}}
\newglossaryentry {AJ} {name={AJ}, description={The Astronomical Journal}}
\newglossaryentry {APC} {name={APC}, description={activities, projects, or state of the profession considerations - wrt. the decadal survey}}
\newglossaryentry {API} {name={API}, description={Application Programming Interface.  Usually this is either "web API" (meaning how you access/update data via http) or "software API" (meaning how you call the function/class/etc in a particular programming language or library), although often only "API" is used and the prefix is implicit.}}
\newacronym {APL} {APL} {Apache Public License}
\newglossaryentry {ATLAS} {name={ATLAS}, description={The Asteroid Terrestrial-impact Last Alert System}}
\newglossaryentry {AURA} {name={AURA}, description={Association of Universities for Research in Astronomy}}
\newglossaryentry {B} {name={B}, description={Byte (8 bit)}}
\newacronym {CADC} {CADC} {Canadian Astronomy Data Centre}
\newglossaryentry {CAOM} {name={CAOM}, description={Common Archive Observation Model \url{http://www.opencadc.org/caom2/}}}
\newglossaryentry {CI} {name={CI}, description={\gls{cyberinfrastructure}}}
\newacronym {CMB} {CMB} {Cosmic Microwave Background}
\newacronym {CPU} {CPU} {Central Processing Unit}
\newacronym {CS} {CS} {Computer Science}
\newglossaryentry {CSSI} {name={CSSI}, description={Cyberinfrastructure for Sustained Scientific Innovation  \url{https://www.nsf.gov/pubs/2019/nsf19548/nsf19548.htm}}}
\newglossaryentry {Citizen Science} {name={Citizen Science}, description={- Amanda, Arfon, Meg?,}}
\newacronym {DES} {DES} {Dark Energy Survey}
\newacronym {DESI} {DESI} {Dark Energy Spectroscopic Instrument}
\newglossaryentry {DIBBs} {name={DIBBs}, description={Data Infrastructure Building Blocks}}
\newglossaryentry {DKIST} {name={DKIST}, description={Daniel K. Inouye Solar Telescope (formerly the Advanced Technology Solar Telescope, ATST)}}
\newacronym {DM} {DM} {Data Management}
\newacronym {DOE} {DOE} {Department Of Energy}
\newglossaryentry {DOI} {name={DOI}, description={Digital Object Identifier \url{https://www.doi.org/}}}
\newglossaryentry {DVCS} {name={DVCS}, description={Distributed Version Control System, a form of \gls{version control} where the complete codebase - including its full history - is mirrored on every developer's computer}}
\newglossaryentry {Docker} {name={Docker}, description={A popular implementation of \gls{container} technology.}}
\newacronym {ELT} {ELT} {Extremely Large Telescope}
\newglossaryentry {EPO} {name={EPO}, description={Education and Public Outreach}}
\newacronym {ESA} {ESA} {European Space Agency}
\newacronym {ESAC} {ESAC} {European Space Astronomy Centre}
\newacronym {EU} {EU} {European Union}
\newglossaryentry {FITS} {name={FITS}, description={Flexible Image Transport System,  is an open standard defining a digital file format useful for storage, transmission and processing of data. Files are formatted as tables or \gls{2D} images}}
\newglossaryentry {FORCE11} {name={FORCE11}, description={FORCE11 is a community of scholars, librarians, archivists, publishers and research funders interested in the Future of Research Communications and e-Scholarship}}
\newglossaryentry {FPGA} {name={FPGA}, description={Field Programmable Gate Array, an integrated circuit which is fairly easily configurable.}}
\newglossaryentry {GB} {name={GB}, description={Gigabyte}}
\newglossaryentry {GNU} {name={GNU}, description={GNU's Not Unix! An operating system and an extensive collection of free computer software}}
\newacronym {GPL} {GPL} {GNU Public License}
\newacronym {GW} {GW} {Gravity Wave}
\newacronym {HPC} {HPC} {High Performance Computing}
\newacronym {HTC} {HTC} {High Throughput  Computing}
\newglossaryentry {IAM} {name={IAM}, description={Identity and Access Management}}
\newglossaryentry {IDL} {name={IDL}, description={Interactive Data Language, a programming language used for data analysis. Harris Geospatial \footnote{\url{https://www.harrisgeospatial.com/Software-Technology/IDL}}}}
\newglossaryentry {IPAC} {name={IPAC}, description={No longer an acronym; science and data center at Caltech}}
\newacronym {IR} {IR} {Infra Red}
\newglossaryentry {IRAF} {name={IRAF}, description={Image Reduction and Analysis Facility,  a collection of \gls{software} written at the National Optical Astronomy Observatory (\gls{NOAO}) geared towards the reduction of astronomical images in pixel array form.}}
\newglossaryentry {IRSA} {name={IRSA}, description={Infrared Science Archive}}
\newglossaryentry {ITAR} {name={ITAR}, description={International Traffic in Arms Regulations}}
\newacronym {IUSE} {IUSE} {Improving Undergraduate \gls{STEM} Education}
\newglossaryentry {IVOA} {name={IVOA}, description={International Virtual-Observatory Alliance}}
\newglossaryentry {JWST} {name={JWST}, description={James Webb Space Telescope (formerly known as NGST)}}
\newglossaryentry {LIGO} {name={LIGO}, description={The Laser Interferometer Gravitational-Wave Observatory}}
\newglossaryentry {LISA} {name={LISA}, description={Laser Interferometer Space Antenna - \gls{ESA} mission for 2030's}}
\newacronym {LSST} {LSST} {Large Synoptic Survey Telescope}
\newglossaryentry {LSSTC} {name={LSSTC}, description={LSST Corporation, a not for profit organisation associated with LSST}}
\newglossaryentry {LUVOIR} {name={LUVOIR}, description={The Large UV/Optical/IR Surveyor - concept mission.}}
\newglossaryentry {MAST} {name={MAST}, description={Mikulski Archive for Space Telescopes}}
\newglossaryentry {MCMC} {name={MCMC}, description={Markov Chain Monte Carlo, a class of algorithms for sampling from a probability distribution.}}
\newglossaryentry {ML} {name={ML}, description={Machine Learning (see also \gls{AI})}}
\newacronym {MSE} {MSE} {Maunakea Spectroscopic Explorer}
\newacronym {NAS} {NAS} {Neural Architecture Search}
\newglossaryentry {NASA} {name={NASA}, description={National Aeronautics and Space Administration}}
\newglossaryentry {NASA ROSES} {name={NASA ROSES}, description={Research Opportunities in Earth and Space Science}}
\newglossaryentry {NGSS} {name={NGSS}, description={Next Generation Science Standards \url{https://www.nextgenscience.org/}}}
\newglossaryentry {NGVLA} {name={NGVLA}, description={Next Generation Very Large Array \url{https://science.nrao.edu/futures/ngvla}}}
\newacronym {NIR} {NIR} {Near Infra Red}
\newglossaryentry {NOAO} {name={NOAO}, description={National Optical Astronomy Observatories (USA)}}
\newacronym {NSF} {NSF} {National Science Foundation}
\newacronym {NSTA} {NSTA} {National Science Teachers Association}
\newacronym {NYU} {NYU} {New York University}
\newglossaryentry {ODBC} {name={ODBC}, description={Open DataBase Connectivity, a standard \gls{API} for \gls{SQL} databases.}}
\newacronym {OS} {OS} {Operating System}
\newglossaryentry {OpenEXR} {name={OpenEXR}, description={a high dynamic range raster file format, released as an open standard along with a set of \gls{software} tools created by Industrial Light \& Magic (ILM) \url{http://www.openexr.com/index.html}}}
\newglossaryentry {PASP} {name={PASP}, description={Publications of the Astronomical Society of the Pacific}}
\newglossaryentry {PB} {name={PB}, description={PetaByte}}
\newacronym {PDF} {PDF} {Probability Density Function}
\newglossaryentry {PHP} {name={PHP}, description={a popular general-purpose scripting language that is especially suited to web development.}}
\newacronym {PI} {PI} {Principle Investigator}
\newglossaryentry {PLATO} {name={PLATO}, description={PLAnetary Transits and Oscillations of stars, the third medium-class mission in \gls{ESA}'s Cosmic Vision programme.}}
\newglossaryentry {PSF} {name={PSF}, description={Point Spread Function,  describes the response of an imaging system to a point source or point object.}}
\newglossaryentry {Pan-STARRS} {name={Pan-STARRS}, description={Panoramic Survey Telescope and Rapid Response System}}
\newglossaryentry {S3} {name={S3}, description={Structured, imperative high level computer programming language, used as implementation language for the Virtual Machine Environment (\gls{VME}) operating system}}
\newacronym {SDSS} {SDSS} {Sloan Digital Sky Survey}
\newacronym {SKA} {SKA} {Square Kilometer Array}
\newglossaryentry {SQL} {name={SQL}, description={Structured Query Language, for interrogating relation databases}}
\newglossaryentry {STEM} {name={STEM}, description={Science, Technology, Engineering and Math}}
\newacronym {TAP} {TAP} {Table Access Protocol}
\newglossaryentry {TB} {name={TB}, description={TeraByte}}
\newglossaryentry {TESS} {name={TESS}, description={Transiting Exoplanet Survey Satellite,  a space telescope for \gls{NASA}'s Explorer program}}
\newacronym {TMT} {TMT} {Thirty Meter Telescope}
\newglossaryentry {TPU} {name={TPU}, description={Tensor Processing Unit , a proprietary type of processor designed by Google in 2016 for use with neural networks and in machine learning projects}}
\newglossaryentry {UA} {name={UA}, description={University of Arizona}}
\newacronym {UK} {UK} {United Kingdom}
\newacronym {US} {US} {United States}
\newacronym {UV} {UV} {Ultra Violet}
\newacronym {VME} {VME} {Virtual Machine Environment}
\newacronym {VO} {VO} {Virtual Observatory}
\newglossaryentry {WFIRST} {name={WFIRST}, description={Wide Field Infrared Survey Telescope}}
\newacronym {ZTF} {ZTF} {Zwicky Transient Facility}
\newglossaryentry {cloud} {name={cloud}, description={A visible mass of condensed water vapor floating in the atmosphere, typically high above the ground or in interstellar space acting as the birthplace for stars.  Also a way of computing (on other peoples computers leveraging their services and availability).}}
\newglossaryentry {cold storage} {name={cold storage}, description={Data moved to \gls{cold storage} means data moved to cheaper slower storage such as tape. The assumption is this is no longer accessed frequently.}}
\newglossaryentry {community software} {name={community software}, description={Software developed for and shared among a large group of relatively like-minded users (e.g. astronomers). Typically, but not necessarily, \gls{open source software} and \gls{open development}-based.}}
\newglossaryentry {container} {name={container}, description={A \gls{container} is a \gls{software} package that contains everything the \gls{software} needs to run. This includes the executable program as well as system tools, libraries, and settings. ... For example, a \gls{container} that includes \gls{PHP} and MySQL can run identically on both a Linux computer and a Windows machine.}}
\newglossaryentry {cyberinfrastructure} {name={cyberinfrastructure}, description={Sometimes denoted \gls{CI}, A term first used by the \gls{US} National Science Foundation (\gls{NSF}), and it typically is used to refer to information technology systems that provide particularly powerful and advanced capabilities.}}
\newglossaryentry {git} {name={git}, description={The most widely used \gls{DVCS} software}}
\newglossaryentry {interoperability} {name={interoperability}, description={the ability of systems or \gls{software} to exchange and make use of information between them.}}
\newglossaryentry {open development} {name={open development}, description={A process for developing \gls{software} that emphasizes all code contribution and decision-making be done in the open, available to as wide a group as possible (This usually means anyone with internet access).}}
\newglossaryentry {open source software} {name={open source software}, description={Open source \gls{software} is a type of \gls{software} in which source code is released under a license in which the copyright holder grants users the rights to study, change, and distribute the \gls{software} to anyone and for any purpose. Note that this is \emph{not} necessarily the same as open to contribution (see \gls{open development}).}}
\newglossaryentry {parquet} {name={parquet}, description={Parquet File Format Hadoop. Parquet, an open source file format for Hadoop. Parquet stores nested data structures in a flat columnar format. Compared to a traditional approach where data is stored in row-oriented approach, \gls{parquet} is more efficient in terms of storage and performance.}}
\newglossaryentry {reproducibility} {name={reproducibility}, description={(this one should have many definitions and we have to say WHICH version we are talking about) The ability to combine the same code and data and get the same result, or the ability to use the same code with different data to enforce a result, or there may be others}}
\newglossaryentry {software} {name={software}, description={The programs and other operating information used by a computer.}}
\newglossaryentry {version control} {name={version control}, description={The management of changes to documents, computer programs, and other collections of information. Changes are usually identified by a number or letter code. Each revision is associated with a timestamp and the person making the change. Revisions can be compared, restored, and merged}}


==> atabAgency.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{Agency recommendations. \label{tab:recAgency1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:datalowbar]{{\textbf \tiny REC-2}  Eliminate barriers to public data access }&Data Management &Medium  \\ 
\hyperref[rec:dataprop]{{\textbf \tiny REC-3}  Proprietary data time scales should be limited, and all datasets should be eventually made publicly available }&Data Management &Short  \\ 
\hyperref[rec:datapreserve]{{\textbf \tiny REC-4}  Long-term data preservation of datasets }&Data Management &Long  \\ 
\hyperref[rec:cbra]{{\textbf \tiny REC-5}  Develop a community wide architecture supporting Science as a Service }&Technology &Long  \\ 
\hyperref[rec:fundops]{{\textbf \tiny REC-7}  Enable support for full mission life cycle including long-term data products  }&Technology &Short  \\ 
\hyperref[rec:opspractices]{{\textbf \tiny REC-8}  Improve long-term \gls {software} and service support }&Technology &Short  \\ 
\hyperref[rec:cmdeploy]{{\textbf \tiny REC-9}  Fund cross-mission deployment }&Technology &Medium  \\ 
\hyperref[rec:swmoney1]{{\textbf \tiny REC-10}  Funding for \gls{software} development in existing grant programs }&Software &Long  \\ 
\hyperref[rec:swmoney2]{{\textbf \tiny REC-11}  Funding for sustaining core astronomical ``community infrastructure'' projects }&Software &Medium  \\ 
\hyperref[rec:swecoplan]{{\textbf \tiny REC-12}  Cultivating a sustainable research \gls {software} ecosystem }&Software &Short  \\ 
\hyperref[rec:algmodels]{{\textbf \tiny REC-13}  Create funding models and programs to support the development of advanced algorithms and statistical methods specifically targeted to the astronomy domain }&Analysis &Medium  \\ 
\hyperref[rec:algconnect]{{\textbf \tiny REC-15}  Promote interdisciplinary collaboration between institutions, fields, and industry }&Analysis &Long  \\ 
\hyperref[rec:algeducation]{{\textbf \tiny REC-16}  Develop an open educational curriculum and principles for workforce training in both algorithms and statistics }&Analysis &Medium  \\ 
\hyperref[rec:algpub]{{\textbf \tiny REC-17}  Encourage, support, and require open publication and distribution of algorithms }&Analysis &Short  \\ 
\hyperref[rec:wc3]{{\textbf \tiny REC-18}  Programs to cultivate the next generation }&Workforce &Long  \\ 
\hyperref[rec:wc5]{{\textbf \tiny REC-20}  Long-term curation of materials }&Workforce &Long  \\ 
\hyperref[rec:wcfundpartner]{{\textbf \tiny REC-21}  Funding for innovative partnerships }&Workforce &Medium  \\ 
\hyperref[rec:wc1]{{\textbf \tiny REC-23}  Training activities and materials }&Workforce &Short  \\ 
\hyperref[rec:wcFund]{{\textbf \tiny REC-27}  Support long-term technical capacity }&Workforce &Medium  \\ 
 \hline
\end{longtable} \normalsize


==> atabAstronomer.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{Astronomer recommendations. \label{tab:recAstronomer1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:datastand]{{\textbf \tiny REC-1}  Adopt common data models throughout the astronomical community }&Data Management &Short  \\ 
\hyperref[rec:dataprop]{{\textbf \tiny REC-3}  Proprietary data time scales should be limited, and all datasets should be eventually made publicly available }&Data Management &Short  \\ 
\hyperref[rec:opspractices]{{\textbf \tiny REC-8}  Improve long-term \gls {software} and service support }&Technology &Short  \\ 
\hyperref[rec:swmoney2]{{\textbf \tiny REC-11}  Funding for sustaining core astronomical ``community infrastructure'' projects }&Software &Medium  \\ 
\hyperref[rec:swecoplan]{{\textbf \tiny REC-12}  Cultivating a sustainable research \gls {software} ecosystem }&Software &Short  \\ 
\hyperref[rec:algmodels]{{\textbf \tiny REC-13}  Create funding models and programs to support the development of advanced algorithms and statistical methods specifically targeted to the astronomy domain }&Analysis &Medium  \\ 
\hyperref[rec:discengine]{{\textbf \tiny REC-14}  Build automated discovery engines }&Analysis &Long  \\ 
\hyperref[rec:algconnect]{{\textbf \tiny REC-15}  Promote interdisciplinary collaboration between institutions, fields, and industry }&Analysis &Long  \\ 
\hyperref[rec:algeducation]{{\textbf \tiny REC-16}  Develop an open educational curriculum and principles for workforce training in both algorithms and statistics }&Analysis &Medium  \\ 
\hyperref[rec:algpub]{{\textbf \tiny REC-17}  Encourage, support, and require open publication and distribution of algorithms }&Analysis &Short  \\ 
\hyperref[rec:wc6]{{\textbf \tiny REC-22}  Software training as part of science curriculum }&Workforce &Medium  \\ 
 \hline
\end{longtable} \normalsize


==> atabEducator.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{Educator recommendations. \label{tab:recEducator1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:wc6]{{\textbf \tiny REC-22}  Software training as part of science curriculum }&Workforce &Medium  \\ 
 \hline
\end{longtable} \normalsize


==> atabManager.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{Manager recommendations. \label{tab:recManager1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:datapreserve]{{\textbf \tiny REC-4}  Long-term data preservation of datasets }&Data Management &Long  \\ 
\hyperref[rec:swecoplan]{{\textbf \tiny REC-12}  Cultivating a sustainable research \gls {software} ecosystem }&Software &Short  \\ 
\hyperref[rec:algconnect]{{\textbf \tiny REC-15}  Promote interdisciplinary collaboration between institutions, fields, and industry }&Analysis &Long  \\ 
\hyperref[rec:wcA]{{\textbf \tiny REC-25}  Recognize \gls {software} as part of the career path }&Workforce &Short  \\ 
 \hline
\end{longtable} \normalsize


==> atabTechnologist.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{Technologist recommendations. \label{tab:recTechnologist1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:datastand]{{\textbf \tiny REC-1}  Adopt common data models throughout the astronomical community }&Data Management &Short  \\ 
\hyperref[rec:cbra]{{\textbf \tiny REC-5}  Develop a community wide architecture supporting Science as a Service }&Technology &Long  \\ 
\hyperref[rec:coloc]{{\textbf \tiny REC-6}  Enable new scales of research through data co-location }&Technology &Medium  \\ 
\hyperref[rec:opspractices]{{\textbf \tiny REC-8}  Improve long-term \gls {software} and service support }&Technology &Short  \\ 
\hyperref[rec:swmoney2]{{\textbf \tiny REC-11}  Funding for sustaining core astronomical ``community infrastructure'' projects }&Software &Medium  \\ 
\hyperref[rec:discengine]{{\textbf \tiny REC-14}  Build automated discovery engines }&Analysis &Long  \\ 
 \hline
\end{longtable} \normalsize


==> atabUniversity.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\tiny \begin{longtable} { p{0.78\textwidth}  p{0.13\textwidth}  p{0.09\textwidth} } 
\caption{University recommendations. \label{tab:recUniversity1}}\\ 
\hline 
\textbf{Recommendation }&\textbf{Area }&\textbf{Term } \\ \hline
\hyperref[rec:wc6]{{\textbf \tiny REC-22}  Software training as part of science curriculum }&Workforce &Medium  \\ 
\hyperref[rec:wcB]{{\textbf \tiny REC-26}  Partnerships to support data science staff }&Workforce &Medium  \\ 
 \hline
\end{longtable} \normalsize


==> audtabs.tex <==
% DO NOT EDIT - this is generated by makeTable.py
\input{atabAstronomer.tex}
\input{atabManager.tex}
\input{atabUniversity.tex}
\input{atabAgency.tex}
\input{atabEducator.tex}
\input{atabTechnologist.tex}


==> authors_new.tex <==
% Author list file generated with: mkauthlist.py UNKNOWN 
% mkauthlist.py --sort -c none Authorlist_Petabytes - Authors.csv 

%%%%%%
% Authors

Brian~Nord
Fermi National Accelerator Laboratory}
\affiliation{Kavli Institute of Cosmological Physics, University of Chicago}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago}
\author{Andrew~J.~Connolly}
\affiliation{DIRAC Institute, Department of Astronomy, University of Washington}
\author{Jaime~Kinney}
\affiliation{Google Inc.}
\author{Jeremy~Kubic}
\affiliation{Google Inc.}
\author{Gautaum~Narayan}
\affiliation{Space Telescope Science Institute}
\author{Joshua~E.~G.~Peek}
\affiliation{Space Telescope Science Institute}
\affiliation{Department of Physics \& Astronomy, The Johns Hopkins University}
\author{Chad~Schafer}
\affiliation{Carnegie Mellon University}
\author{Erik~J.~Tollerud}
\affiliation{Space Telescope Science Institute}


%%%%%%
% Endorsers

\author{Camille~Avestruz}
\affiliation{Enrico Fermi Institute, The University of Chicago}%, Chicago, IL 60637 U.S.A.}
\affiliation{Kavli Institute of Cosmological Physics, University of Chicago}

\author{G.~Jogesh~Babu}
\affiliation{Center for Astrostatistics}

\author{Simon~Birrer}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles}%, CA 90095, USA}

\author{Douglas~Burke}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian}

\author{Jo\~ao~Caldeira}
\affiliation{Fermi National Accelerator Laboratory}

\author{Douglas~A.~Caldwell}
\affiliation{SETI Institute}

\author{Joleen~K.~Carlberg}
\affiliation{Space Telescope Science Institute}

\author{Yen-Chi~Chen}
\affiliation{Department of Statistics, University of Washington}

\author{Chuanfei~Dong}
\affiliation{Princeton University}

\author{Eric~D.~Feigelson}
\affiliation{Department of Astronomy \& Astrophysics, Penn State University}
\affiliation{Center for Astrostatistics, Penn State University}

\author{V.~Zach~Golkhou}
\affiliation{DIRAC Institute, Department of Astronomy, University of Washington}%, 3910 15th Avenue NE, Seattle, WA 98195, USA}

\author{Vinay~Kashyap}
\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian}

\author{T.~S.~Li}
\affiliation{Fermi National Accelerator Laboratory}

\author{Luisa~Lucie-Smith}
\affiliation{Department of Physics \& Astronomy, University College London}%, Gower Street, London WC1E 6BT, UK}

\author{Kaisey S. Mandel}
\affiliation{University of Cambridge}

\author{Adam~A.~Miller}
\affiliation{CIERA, Northwestern University}
\affiliation{The Adler Planetarium}

\author{Priyamvada~Natarajan}
\affiliation{Department of Astronomy, Yale University}%, New Haven, CT 06511 USA}

\author{Michelle~Ntampaka}
\affiliation{Harvard Data Science Initiative, Harvard University}%, Cambridge, MA 02138, USA}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian}

\author{Andy~Ptak}
\affiliation{NASA/Goddard Space Flight Center}

\author{David~Rapetti}
\affiliation{CASA, Department of Astrophysical \& Planetary Science, University of Colorado, Boulder; NASA Ames Research Center}%, CO 80309, USA}

\author{Lior~Shamir}
\affiliation{Department of Computer Science, Kansas State University}%, Manhattan, KS}

\author{Aneta~Siemiginowska}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian}

\author{Brigitta~M.~Sip\H{o}cz}
\affiliation{DIRAC Institute, Department of Astronomy, University of Washington}

\author{Arfon~M.~Smith}
\affiliation{Space Telescope Science Institute}

\author{Nhan~Tran}
\affiliation{Fermi National Accelerator laboratory}

\author{Ricardo~Vilalta}
\affiliation{Department of Computer Science, University of Houston}

\author{Lucianne~M.~Walkowicz}
\affiliation{The Adler Planetarium}
\affiliation{LSSTC Data Science Fellowship Program}

\author{John~ZuHone}
\affiliation{Smithsonian Astrophysical Observatory}










==> authors_old.tex <==

% \author{Amanda~E.~Bauer}
% \affiliation{Large Synoptic Survey Telescope (LSST/AURA)}
% \author{Eric C.~Bellm}
% \affiliation{LSST}
% \affiliation{DIRAC Institute, Department of Astronomy, University of Washington}
% \author{Adam~S.~Bolton}
% \affiliation{NOAO}
% \author{Surajit~Chaudhuri}
% \affiliation{Microsoft Research}

% \author{Kelle~L.~Cruz}
% \affiliation{Hunter College, City University of New York}
% \affiliation{American Museum of Natural History}
% \affiliation{Center for Computational Astrophysics, Flatiron Institute}
% \author{Vandana~Desai}
% \affiliation{Caltech/IPAC}
% \author{Alex~Drlica-Wagner}
% \affiliation{Fermi National Accelerator Laboratory}
% \affiliation{Kavli Institute of Cosmological Physics, University of Chicago}
% \author{Frossie~Economou}
% \affiliation{Large Synoptic Survey Telescope (LSST/AURA)}
% \author{Niall~Gaffney}
% \affiliation{Texas Advanced Computing Center}
% \author{J.~Kavelaars}
% \affiliation{National Research Council of Canada}

% \author{Ting~S.~Li}
% \affiliation{Fermi National Accelerator Laboratory}
% \affiliation{Kavli Institute of Cosmological Physics, University of Chicago}
% \author{B.~Lundgren}
% \affiliation{University of North Carolina Asheville}
% \author{R.~Margutti}
% \affiliation{Northwestern University}

% \author{Dara~J.~Norman}
% \affiliation{NOAO}
% \author{W.~O'Mullane.}
% \affiliation{Large Synoptic Survey Telescope (LSST/AURA)}
% \author{S.~Padhi}
% \affiliation{Amazon Web Services}

% \author{Megan ~E.~Schwamb}
% \affiliation{Gemini Observatory}
% \author{Arfon~M.~Smith}
% \affiliation{Space Telescope Science Institute}
% \author{Alexander~S.~Szalay}
% \affiliation{Department of Computer Science, The Johns Hopkins University}
% \affiliation{Department of Physics \& Astronomy, The Johns Hopkins University}

% \author{Anne-Marie~Weijmans}
% \affiliation{School of Physics and Astronomy, University of St Andrews}


==> caveat.tex <==
\noindent\textbf{Note:}
If you have come directly to this chapter we suggest you please read at least the Introduction in \secref{sec:intro} before delving further.
\newline
%\newline


==> conclusion.tex <==
\section{Conclusion }
\label{sec:conclusion}

We had a good opportunity to think about a range of topics which have been detailed in this document. Several \gls{APC} white papers will be published using this  as a basis.
If you are interested in contributing to or endorsing \href{white papers on these topics sign up here}{https://tinyurl.com/y2ksemp2}\footnote{ \url{https://tinyurl.com/y2ksemp2}}  or contact the authors listed in this document.
We do not intend this to be the solution to all issues rather a discussion of potential ways forward for the next decade.
We shall host a \href{https://petabytestoscience.github.io/}{third and final workshop}\footnote{\url{https://petabytestoscience.github.io/}} in October 2019 which will explore practical approaches to dealing with some of the recommendations raised here.


==> data.tex <==
\section{Data Management}\label{sec:data}
\noindent\Contributors{Anne-Marie Weijmans <\mail{amw23@st-andrews.ac.uk}>, JJ Kavelaars <\mail{JJ.Kavelaars@nrc-cnrc.gc.ca}>, Surajit Chaudhuri, Vandana Desai, Jamie Kinney, William O'Mullane, Alex Szalay}

\bigskip
\input{caveat}

In this section we recognize two of the main challenges related to data management in the next decade:

\begin{itemize}
    \item Big Data: datasets will be of such large volume, that moving them across individual data repositories is not practical. This will affect the way that we interact with data, and has the risk that some users will be excluded from access to large datasets. (See also \secref{sec:coloc})
    \item Time Domain: datasets will contain a time domain element, i.e. will contain data of the same part of the sky obtained at different time intervals. This will put challenges on current visualisation and discovery tools.
\end{itemize}




To address these two challenges, we make the following recommendations:

    \nrec{Data Management}{Astronomer, Technologist}{Short}{datastand}{Adopt common data models throughout the astronomical community}{The astronomical community should work towards a common data model. This will allow astronomers to concentrate on scientific exploration of datasets, without having to worry about data formats and structures}
    \nrec{Data Management}{Agency}{Medium}{datalowbar}{Eliminate barriers to public data access}{Astronomical public datasets should be accessible to everyone, and everyone should have the opportunity to contribute to astronomical public datasets}
   \nrec{Data Management}{Agency, Astronomer}{Short}{dataprop}{Proprietary data time scales should be limited, and all datasets should be eventually made publicly available}{To maximize scientific output, and allow wider-community access of centralized funded projects, all astronomical datasets should be made publicly available and accessible after an appropriate but short proprietary time limit}
    \nrec{Data Management}{Agency, Manager}{Long}{datapreserve}{Long-term data preservation of datasets}{Long-term data preservation and management should be an integral part of community-wide project planning}

%    brian.d.nord: should there be example solutions for the near-term that ground the long-term recommendations?
  %  \item \rec{datastand2}{Common data exchange and storage formats}{The astronomical community should converge to common data exchange and data storage formats, preferably based on industry standards, to allow access and analysis of big datasets and curation of time domain data}

We discuss these recommendations in more detail in the sections below.

\subsection{Interoperability}

% https://docs.google.com/document/d/1fANclpby13KX67WrfFIy60MLt1zs25Ea32Y3Zu7wiuk/edit --> google doc with original text and questions that led to this subsection

In the 2020s, new datasets such as \gls{LSST}, \gls{WFIRST}, and Euclid hold enormous science promise. Realizing this potential for transformative science presents a number of challenges for data management. As we outlined above: the main challenges are the volumes of the data, as well as the additional dimension that time domain observations will bring to these large datasets.


\subsubsection{Common observation models}

{\em Data centers should adopt a common observation model (\recref{rec:datastand}}). A common observation model is a set of standard metadata parameters that can be used to describe any astronomical dataset. The widespread adoption of a common observation model has many advantages, outlined below.

The large volume of data in the 2020s implies that re-processing these data will incur high cost, thus increasing sharply the importance of a common data model that can serve as the basis for information exchange and reuse. International Virtual Observatory Alliance \gls{IVOA} is on the way to adopting the Common Archive Observation Model (\gls{CAOM}) for images. It has already been adopted by a number of large archives, including the \gls{CADC}, the \gls{ESAC}, the Mikulski Archive for Space Telescopes (\gls{MAST}), and the \gls{NASA}/\gls{IPAC} Infrared Science Archive (\gls{IRSA}).

Effective re-use of data requires careful, ongoing curation of this metadata model. This includes both preserving the expertise and context of what the nuances of a particular dataset are, but also periodically updating metadata to conform to new standards and meet new use cases. For example, astrometry of old datasets may need to be updated to support real-time querying/matching/aligning/jointly processing for time domain studies.

\subsubsection{Data storage}
%\WOM{Quite similar to Section \ref{sec:coloc}}

{\em Data Centers should adopt industry standards for data storage when possible,} see also \secref{sec:coloc}.
Perhaps the most obvious challenge is simply storing the data. The large volumes mean efficiency in storage representation is important.

We recommend that data centers leverage ‘off-the-shelf’, open data management services, tools, and technologies that have been developed by industry.
Moving to industry standards for things like images allow us to leverage new technologies such as the ability to stream and operate remotely on {\em objects} using standard tools.
File systems as we know them will not be the most appropriate storage model at petascale levels.
Alternatives include the use of \gls{cloud} object stores, \gls{cloud} compute, ‘big data native’ formats such as Apache \gls{parquet} and \gls{OpenEXR}, and cloud-optimized \gls{FITS} (see \gls{cloud} optimized GeoTIFF as an example https://www.cogeo.org). Traditional astronomy file formats (e.g. \gls{FITS}) should be used as they were originally intended, for transport only. That being said, one big advantage of \gls{FITS} files is their ability to co-package meta-data, while e.g. for Parquet there are only limited options to have meta-data included directly with the data. Data and meta-data should be managed together to not lose efficiency in analysis performance.


\subsubsection{Eliminating file systems}

{\em The community should develop a flexible suite of application program interfaces to abstract the file system.}

The previous recommendation calls for using storage formats that are optimized for the \gls{cloud}, in order to meet the challenge of “Big Data” storage. This also implies that the current often used practice of storing files and file systems locally on astronomers' laptops of analysis will have to change to this more global approach of accessing and analyzing data remotely. To avoid a difficult transition for many individual astronomers, global file structures and formats should be abstracted by two layers of application program interfaces (\gls{API}s). The bottom layer consists of a limited set of (\gls{VO})-based APIs implemented by data centers. We recommend that data centers implement a critical set of core \gls{VO} \gls{API}s, including cone search, image search, spectral search, \gls{TAP}, the standardized language used to report observations of astronomical events \gls{VO}Event, and Ephemeris Lookup (still to be adopted by the \gls{IVOA}). Other \gls{VO} standard protocols have become obsolete, and should not be implemented (e.g. \gls{VO}Space in favor of \gls{S3}). The top layer consists of user-facing \gls{API}s developed by the community to “hide” the file formats from the user. In the 2020s, this top layer should focus on Python. However, lightweight \gls{API}s can be built in other languages as community needs dictate.

%Who should pay for this?



\subsubsection{Interoperable science platforms}

{\em Data Centers should provide a set of interoperable science platforms.}

A science platform provides users with access to compute and analytic services close to the datasets of interest. With new astronomy survey datasets measured in petabytes, it is quickly becoming infeasible to copy entire datasets to another location for analysis. At the same time, it is increasingly common for researchers to leverage big data and inefficient parallel compute technologies to analyze large subsets, if not entire datasets. Cloud services provided by commercial organizations and \gls{DOE}/\gls{NSF}-funded High Performance Computing (\gls{HPC}) centers offer both the scale of compute resources and the networking infrastructure required to analyze these datasets using modern techniques.  Furthermore, by physically co-locating datasets, we make it possible for researchers to conduct investigations that incorporate data from multiple mission archives. Therefore, we recommend that the \gls{DOE}, \gls{NSF}, and other funding agencies encourage data archives to be physically stored and perhaps co-located in facilities which are accessible to the global research community and which provide the compute and higher-level analytical services that will be used to analyze these datasets at scale.





\subsection{Lowering the barriers to public data access}


{\em Projects should eliminate barriers to public data access (\recref{rec:datalowbar}), and limit the proprietary data time scale (\recref{rec:dataprop}).}
To make maximal use of astronomical datasets, every astronomer should have access to these datasets, and have the tools available to exploit their scientific richness. In the sections below we make suggestions that projects should adopt to ensure that barriers to work with data are removed: we concentrate here on astronomical community (including students), and refer to \secref{sec:epo} for promoting astronomical data with the general public. We also recommend that although proprietary data has its use within the astronomical community (e.g. ensuring that the astronomers and students who invested in collecting and reducing the data have the opportunity to explore the datasets for their science), that these proprietary times are kept short to maximize over-all science output.



\subsubsection{Computational resources}
{\em Projects should make their datasets available for remote data analysis}
As mentioned in the previous section, the big datasets of the next astronomical surveys will be too large to download and store on individual astronomers computing systems (laptops). Projects should therefore ensure that their data is available for remote analysis, and provide opportunities for \gls{cloud} computing. This will ensure that the whole astronomical community will have access to the data, and that lack of large data storage and/or computing facilities will not prevent astronomers from taking part in the scientific exploration of large datasets. We note that \gls{cloud} computing does require reliable internet connections, which for most of the astronomical community will be available, but not necessarily for a more general audience (e.g. schools and individuals in remote areas).



\subsubsection{Documentation}
{\em Projects should allocate sufficient resources and attention to capturing the expertise on collection, processing and interpretation of their data products.}
A dataset is only as strong as its documentation. Without documenting the expertise needed to work with a dataset, scientific analysis based on that data has a high risk of being flawed. Including detailed documentation with data resources is therefore a must.  The documentation that captures the projects expertise should be easily accessible: the documentation should be released at the same time as the datasets. The documentation should be clearly written, with jargon explained and with tutorials and examples for clarification. The documentation should not be aimed at the experts within a project, but be written with inexperienced, new users in mind (e.g. students). There should be a mechanism (e.g. helpdesk, forum), in place to collect feedback and errata, and the documentation should be updated and improved accordingly during the life time of the project. Having excellent documentation does not only lower the barriers of entry to work with large datasets, but will also be invaluable when the project has reached the end of its lifetime, and the datasets will (eventually) go into long-term archiving (see Section~\secref{sec:datapreservation}).


\subsubsection{Professional training}
{\em Training resources on the exploration of large public datasets should be made available for free and on-line.}
To lower barriers for entry further, there should be training resources available for the astronomical community, to ensure that they can explore the richness of large public datasets. These training resources, such as tutorials, demos and notebooks, should be aimed at appropriate levels, as the education needs of a beginning students are different than those of a postdoc or faculty member. These resources should be available and accessible to a large audience, and therefore should be linked to from dataset documentation pages.

%In addition to training resources, we also recommend that %projects implement

% community building around helpdesk/forums, requires critical mass and be supportive, welcoming. International, and allow multiple languages
% still need experts and funding to set this up
% value in partnering with Universities, but don't depend on them: don't exclude astronomers at underpriviliged communities
% have representation on science advisory commitees --> workforce section
% mobile friendly



\subsubsection{Education and Public Outreach}
{\em Data facilities should invest in collaborations with Education and Public Outreach teams.}
Having real astronomical public data available for education and public outreach purposes is a big advantage for developing resources that closely mimic and can even contribute to scientific research.
As outlined in  \secref{sec:epo} the Education and Public Outreach (\gls{EPO}) chapter of this document, we recommend supporting dedicated education and outreach groups with relevant expertise to maximize the impact of \gls{EPO} activities. To work closely with these \gls{EPO} teams, we recommend that  each data facility has at least one team member to liaise with the \gls{EPO} team, and provide input on data requirements for \gls{EPO} activities.


\subsection{Long-term data preservation}
\label{sec:datapreservation} %refereced in technology section

{\em Long-term data preservation and management should be an integral part of community-wide project planning (\recref{rec:datapreserve})}
Data that is actively used will continue to exist in the community: there is a sort of Darwinian selection going on constantly. Expertise is therefore also kept reasonably current while the data are in use. But the implication is that some data will be getting used less and less over time, and at some point is going to be compressed (including documentation and possible email archives) and put into \gls{cold storage} for long term preservation. Catalogs and derived data products could potentially persist in regular use for longer than their source data.

The long term preservation of data is a problem that is not unique to Astronomy or Science, neither in volume nor in characteristics. Such preservation has the following components:
\begin{enumerate}
    \item Ensuring data integrity (no tampering)
    \item Sufficient redundancy so that there is no single point of failure, to ensure data access
    \item Packaging of information that provides “recoverability” of essential information
    \item Funding for such preservation, as well as data format and \gls{software} maintenance.
\end{enumerate}
The first challenge (data integrity) is  a general problem, and  there are many techniques that have been developed in research and in industry to ensure integrity. These include tamper-proof logs and signature based comparison of multiple copies of preserved data including watermarking. We should select a preferred method in astronomy.

The second challenge is met b and perhaps co-located having multiple sites to ensure that there is no single point of failure.  There is a cost vs. “how many failures you can tolerate” trade-off. Offloading this task to multiple vendors of public \gls{cloud} companies is probably the simplest solution. One compelling reason to do that is because they will, due to market pressure, continue to support changing data formats and media as technology change. Through all these, the data should remain accessible, even when in \gls{cold storage}.

The third challenge, which is packaging of information, is most critical and this is where unique aspects of Astronomy are relevant. A data dump in itself is not easy to interpret, especially after several years, when the experts that generated and worked with the data have moved on to other projects. Therefore, it is critical to have good documentation and metadata enrichment. We need to  capture the \emph{expertise} so we may want to compress and store communications such as Slack channels, mailing lists and logs etc. As well as the actual data.
By having such additional catalogs, the “recoverability” of value from preserved data is much enhanced. However, we need to acknowledge that such often more informal and unsorted communication does not replace the need for comprehensive and understandable documentation and tutorials to work with the data. The value of archived communication would be for the (hopefully) rare instances that an issue occurs that is not documented probably, but was discussed on communication channels, and for historic and/or social studies.

Last but not the least, there is the funding question. There are two possible models. First model is to attach a “service fee” to every funded project to support ongoing high quality documentation. Alternatively, funding may be requested as we near end of the project. The payment model, especially to \gls{cloud} providers, could be fashioned like what is done for title insurance for home purchases – an one-time payment for a fixed number of years

%%%% The following text is all commented out: contains older versions, musings and text that was cut out.  %%%%


\begin{comment}

Data sets of future missions like \gls{LSST}, \gls{WFIRST} and Euclid will have significant volumes, which asks for efficient storage. It also implies that reprocessing of data will incur high costs in terms of computational resources, which highlight the importance of a common data model which can serve as the basis for information exchange and reuse. For efficient storage, we should leverage ‘off the shelf’ data management services (e.g. object stores, compute) and tools/technologies that have been developed in the commodity computing/commercial \gls{cloud}
We should leverage ‘big data native’ formats such as Apache Parquet, \gls{OpenEXR}.
\gls{cloud}-optimized \gls{FITS} (see \gls{cloud} optimized GeoTIFF as an example https://www.cogeo.org),

Using data formats that are Time Domain
Curation of existing data becomes increasingly important. This includes both preserving expertise/context of what the nuances of a particular dataset are, but also periodically updating metadata e.g. astrometry so that data can be queried/matched/aligned/jointly processed in real time or interactive speed.

\end{comment}


\begin{comment}
\subsection{Temporary: Raf's notes on Time Domain challenges}
Raf: notes for Time-domain \\
Background: Time-domain astronomy is the new frontier of Discovery. We now have the technical capabilities to monitor the night sky in real time and explore the fourth dimension: TIME. This ``observational exercise'' has led to the discovery of new types of phenomena that challenge current notions of physics, and led to the recent landmark discovery of light from a gravitational-wave source. Current and near-future astronomical transient surveys like the Zwicky Transient Facility (\gls{ZTF} led by Caltech, 2018+) and the Large Synoptic Sky Telescope (\gls{LSST}, 2023+) will take this effort to the next level and will generate an unprecedented data stream in terms of volume, variety, and velocity. To succeed in the quest for new phenomena, the challenge is two-pronged: (i) it will be necessary to identify specific targets of interest amidst millions of alerts each night; (ii) we will need very fast identification of notable alerts, ideally within minutes of detection, to enable prompt follow-up observations (spectroscopy and/or observations across the electromagnetic spectrum) that historically led to major discoveries.
To summarize: the challenge is to recognize the interesting transients among thousands of uninteresting sources, and to do it fast!

The problem: Time-domain astronomy is rapidly approaching a breaking point in its ability to quickly identify transient alerts. The traditional approach of spectroscopic classification is clearly not a viable, scalable option (in the \gls{LSST} era, even using all available telescopes, we would only be able to classify a vanishing percentage of transients!). There are two complementary approaches to solve this problem: (1) early light-curve classification; (2) environments (i.e. guessing ``who'' you are from where you live).

Method (1) relies solely on the first few data points of a transient light-curve. Here, the core idea is to develop machine-learning systems to identify the nature of newly detected transients by matching the properties of their early light-curves to known transients. This approach is attractive (and “cheap” in terms of not requiring new data), but suffers from three severe limitations: (1) Acquiring enough light-curve data points to distinguish between different types of transients will require time (one to several days), as there is degeneracy in the early-time behavior of intrinsically different transients. This process makes prompt and reliable identification of transients virtually impossible. (2) Identifying previously unrecognized phenomena by matching their properties to known transients severely limits any possibility of discovering the unknown. (3) Building machine-learning algorithms requires very large training datasets that are currently nonexistent. At present, only a few dozen transients have detailed observations at early times, which is insufficient to develop machine learning models that could effectively classify the diversity of transients that we will encounter. This is especially true for some of the most interesting transients, like counterparts to gravitational-wave triggers, the most luminous, rare supernovae, and tidal stellar disruptions around supermassive black holes.

Method (1) is way more promising when complemented with method (2), which uses contextual information, i.e. information that already exists in astronomical data repositories across the electromagnetic spectrum (from radio waves to gamma-rays, including X-rays, \gls{UV}, optical/\gls{NIR}). The benefits of contextual information to enabling classification are well-known to the community (e.g. stellar disruptions by supermassive black holes only happen at the center of their galaxies, while massive stellar explosions prefer young stellar environments anywhere in galaxies, and supernovae used for cosmology also happen in old stellar populations). Yet, for method (2) to be effective, all catalogs needs to be queried fast, something that at present is just not feasible. The information is there, but not available on the relevant timescales of seconds after alert.

\end{comment}






\begin{comment}
Paraphrasing Frossie's comment: Should address the timeliness of these recommendations? \#3 was recommended in 2010, as Dara said. \#2 sounds an awful lot like the \gls{VO}. What in the coming decade makes this the time to execute? --> this is now addressed by adding that what is new is 1) Big Data and 2) Time Domain
\end{comment}


\begin{comment}
\begin{enumerate}
    \item Agree on a standards body for data management across astronomy.
    \item Lower the barrier for data access and creation for both education and research, for a variety of audiences. [a suggestion that authentication is a solved problem may help lower barrier]
    \item Develop a strategic plan for long-term data preservation,  active curation, documentation, and access as a part of the data and project life cycle. (As recommended in the previous decadal survey)[virtual co-location of data] [eases discovery]
    \item Data analysis services and exploration platforms should be incentivized by the funding agencies to present low barriers to entry to allow the on-going exploitation of data holdings
\end{enumerate}


\subsection{Data Creation and Infrastructure}
\WOM{Does this belong in the technology and infrastructure section?}

Commodity and/or bespoke. Commodity examples: \gls{cloud}, we're tapping into it for our own uses, but not building them --> overlap with infrastructure

Infrastructure to make data available underpinning journal publications. Obligatory now in \gls{UK} and some \gls{EU} countries, as requirements for funding agencies.

Projects need to have a plan for long-term curation after completion of project --> already in 2010

Work with archive systems from beginning of survey. Aware of archive standards

Take away barriers and provide support for those scientists that want to contribute value added catalogs and datasets. Also for \gls{software} and visualisation.


\subsection{Data Accessibility}

Want to make sure that everyone has access, not just put all resources on one program / problem / \gls{PI};  consider the positive effects this would have on under-resourced institutions
Have one platform/format for all the data download/retrieving. Standardized this so that people do not need to learn how to do that for every release/publication.



Access is more than getting but ability to use (Science Ready) and that is a moving target with \gls{PI}s over time.

How to connect with journals for data publication [Niall]? Or what about an ArXiv for data and for \gls{software} [nord]?

Development of standard data access methods this would make long term preservation easier - also we would not need to cycle data out to \gls{cold storage}.

How to keep data up to date? If you google \gls{SDSS}, and find an old data release?


\subsection{Data Longevity}

Measurements of data access, statistics. When time to retire the data?

Archive the documentation! How to use the data and the meta data.

How to archive interfaces?

Changes in data formats?

Make sure we don't carry over unnecessary baggage.

Keep data authentic, avoid hacks / data falsification



\end{comment}



\begin{comment}


\subsection{Telescope - Data Centre interaction}

The following structure is just to organize our thoughts and will be adapted throughout the writing process. Please add your thoughts and bullet points for discussion, where you seem fit, and also feel free to add new subsections! AMW \& JJK

Add your thoughts on this subsection here, also please add bullet points!



\begin{itemize}
    \item Photons to data products: data reduction and data transfer
    \item Interaction with Operations
    \item Data archive and preservation
\end{itemize}



\par (Vandana) I am confused about the definition of "Data Center". Sometimes (often) the place where the data products are generated is not the same as the place where the data are archived. Perhaps a diagram would be useful in this section, tracing the path of the data to the user. Also, are Section 3.1 and 3.2 meant to describe the current state of data flow, while 3.3 suggests changes? If so, that means a reader will have to slog through a lot of boring stuff before they hear any recommendations. Should each major section perhaps have an abstract summarizing recommendations before diving into details? In section 3.3, I imagine that Long-term stewardship should appear first in the list. I'm not sure what the difference is between "Integration of different archives and systems" and "International Interoperability". Is it just national versus international? I don't think \gls{DOI}s should necessarily be linked with Data Preservation, as data can and has been preserved without \gls{DOI}s. They seem to be more about discoverability. I also am not sure how "Data Preservation" is different than "Long-term stewardship". I feel like something addressing the challenges of "Big Data" should be in this list, as well as "Analysis at the Archives" or "Science Platform". Perhaps that is meant to be in the Software \& Service section? In any case, it seems key to "Data Center - User interaction", so perhaps it can be at least cross-referenced? Seems like the role of Virtual Observatory Protocols should be on here, as well, as they are important both for connecting data centers / archives and for user programmatic access.

\subsection{Data Centre- User interaction}

\begin{itemize}
    \item Data access and open data access infrastructure - AMS: I'm vaguely obsessed with the `Principles for Open Scholarly Infrastructures' \footnote{ \url{https://cameronneylon.net/blog/principles-for-open-scholarly-infrastructures/}} which could be something to discuss here.
    \item Data products to science
    \item Team science: sharing data and sharing algorithms and processes
    \item Lowering the barrier for participation (both \gls{LSST} workgroup members and public)
    \begin{itemize}
        \item Collecting feedback from the community (note: overlap with workforce chapter)
        \item helpdesk
        \item tutorials and maintenance of tutorials
        \item data/science centers as places for collecting, organizing, and maintaining \emph{expertise} around data and methods
        \item  scaffolded methods for access \& analysis, tailored to different audiences (e.g. public \& pre-professional audiences don't need to see the \gls{SQL} behind the curtain, \& they may only need smaller, curated subsets of the data)
    \end{itemize}
    \item Contributed data products (value added catalogs) - Integration of those user contributed science catalogs with related products and part of the original survey or data collection.
    \item A path to contributed \emph{services}
    \item Application of user contributed \gls{software} algorithm to produce standard products or coordination between data teams and data centre to ensure products can be distributed.
\end{itemize}

Add your thoughts on this subsection here, also please add bullet points!

\subsection{Data Centre - Future Interactions}

\begin{itemize}
    \item Integration of different archives and systems
    \item International Interoperability
    \item Long-term stewardship
    \item Preserving expertise for working with data
    \item Data Preservation, \gls{DOI}s
    \begin{itemize}
        \item How do we deal with today’s data in 30 years, ?
        \item Alex's \gls{AAS} talk (endowment, libraries?): \footnote{\url{http://www.sdss.jhu.edu/~szalay/powerpoint/szalay-aas-wide-2019.pptx}}
        \item public/private partnership models
    \end{itemize}
    \item Including simulations and synthetic data in this access?
    \item Interoperability of identities (Could be in Infrastructure and technology). OR\gls{CI}D?

\end{itemize}

\end{comment}




==> old_text/Makefile <==
#for dependency you want all tex files  but for acronyms you do not want to include the acronyms file itself.
tex=$(filter-out $(wildcard *glossary.tex) , $(wildcard *.tex))  

DOC=main
SRC= $(DOC).tex
OBJ=$(SRC:.tex=.pdf)

#Default when you type make
all: $(OBJ)

$(OBJ): $(tex) aglossary.tex
	latexmk -bibtex -xelatex -f $(SRC)

#The generateAcronyms.py  script is in lsst-texmf/bin - put that in the path
aglossary.tex :$(tex) myacronyms.txt
	generateAcronyms.py  -g  $(tex) aglossary.tex
	generateAcronyms.py -u -g  $(tex) aglossary.tex

authors.tex: Authorlist_Petabytes\ -\ Authors.csv 
	python3 mkauthlist.py --sort -c none Authorlist_Petabytes\ -\ Authors.csv | grep -v collaboration > authors.tex

clean :
	latexmk -c
	rm *.pdf *.nav *.bbl *.xdv *.snm


glossaries:
	makeglossaries $(DOC)


==> old_text/acknowledgments.tex <==

\subsection*{Acknowledgments}

The workshops in this series were supported by The Kavli Foundation\footnote{\url{https://www.kavlifoundation.org/}}. The Kavli Foundation is dedicated to advancing science for the benefit of humanity, promoting public understanding of scientific research, and supporting scientists and their work.

%A Kavli foundation sponsored workshop on the theme \emph{Petabytes to Science} was held 12$^{th}$ to 14$^{th}$ of February 2019 in Las Vegas.
%The aim of the this workshop was to discuss important trends and technologies which may support astronomy. We also tackled
%how to better shape the workforce for the new trends and how we should approach education and public outreach.
%This document was coauthored during the workshop and edited in the weeks after.
%It comprises the discussions and highlights many recommendations which came out of the workshop.

 

==> old_text/epo.tex <==
\section{A need for dedicated education and outreach expertise
\Contact{Amanda Bauer}}
\Contributors{Amanda E. Bauer <\mail{abauer@lsst.org}>, Britt Lundgren, Meg Schwamb, Brian Nord, Dara J Norman}
\label{sec:epo}

\bigskip
\input{caveat}

%White Paper Abstract here as comment
%There exists a new opportunity in the realm of large surveys and data facilities for online education and outreach activities to have a huge impact on society in the 2020s. In order to meet the public demand for mobile-friendly and intuitive user interfaces, and a discovery space driven by social media, the development of digital activities should be guided by centralized EPO teams who can create, evaluate, and disseminate innovative EPO activities in a way that astronomers can tap into. Astronomers can then contribute to these activities or adapt the products to advance their own outreach efforts. This means that we must commit and dedicate resources to education, outreach, and communication professionals who can provide strategy, oversight, training, and instill best practices to maximize the impact of outreach efforts and increase accessibility of science results within the public field of vision. EPO teams should draw on astronomical expertise, education theory and practice, user interface and user experience skills, software engineering skills, and communication experts. This White Paper will outline some examples of what is currently available and work that needs to be done to maximize the impact of ongoing outreach efforts and elevate society's engagement with the process of scientific discovery in the next decade.

We need to capitalize on positive trends in digital literacy, the increasing use of mobile devices, and a discovery space driven by social media, through the progressive development of online resources in astronomy education and public outreach (\gls{EPO}). The goal for this chapter is to clarify and bolster the multitude of opportunities that exist to develop newly accessible online tools to engage fellow citizens in the era of petabyte-scale astronomy.

Maintaining support for astronomy research relies on our ability to effectively communicate our science and cultivate public excitement and engagement. Historically, strategic programming for astronomy \gls{EPO} in science projects has been an afterthought: the work has primarily been undertaken by astronomers who are passionate about \gls{EPO} but may lack the specific professional skills required to do it effectively at scale.  Moreover, most astronomers are not compensated for their time or rewarded by their efforts in \gls{EPO}. To maximize the public impact of large projects in the petabyte era, we must give professional credit to astronomers who do outreach work and also dedicate resources to full-time personnel to develop, execute, and evaluate modern \gls{EPO} activities.

Traditional means of public engagement (e.g. classroom visits, online videos, public lectures and panels, etc.) have demonstrated their importance and value, and have carved a niche in the landscape of public engagement. However, we have entered a new era of technology and social interaction, which necessitates new modalities for innovative pedagogical techniques, communication, and even scientific exploration. Taking advantage of opportunities of modern technology requires putting in place the appropriate professionals to create and develop the interfaces and connections to curricula that maximize adaptability and use. For example, connecting non-experts with ever larger datasets requires educators who have astronomy domain expertise (to curate and work with datasets) as well as expertise in innovative pedagogical practices.

{\bf In this new era of engagement, \gls{EPO} teams who develop ground-breaking activities and pedagogical frameworks will have started the design process as early as possible (including during construction of new facilities) and will have drawn on a number of areas of expertise: astronomical research methods, educational theory and practice, web development and design, \gls{software} engineering, and multi-modal communication.}

In this chapter, we discuss recommendations and effective practices for advancing astronomy in society through data-driven education and outreach activities for maximizing the impact large observing facilities and data centers will provide. We begin by discussing the creation of accessible online activities (\secref{epo-online}), then identify a range of skills needed to create such activities (\secref{eposkills}), and finally, we establish the benefits of resourcing dedicated \gls{EPO} groups from the earliest stages of astronomy facility planning and including \gls{EPO} as part of the mission of projects (\secref{epogroups}).


\subsection{Create accessible online activities for the public}\label{epo-online}

\nrec{EPO}{Educator, Astronomer}{Short} {epo1}{Create accessible online Activities for the Public}{To maximize the impact of astronomy in society in the rapidly approaching petabyte and exabyte eras, we recommend that projects and data centers develop accessible web interfaces and tools that enable the public to access, explore, and analyze authentic astronomical data at unprecedented scale.}

Many good arguments have been made for enabling non-professionals and students to access and engage with authentic data and professional tools. However, in practice, the increasing complexity of interfaces to large datasets can become a barrier to access and use.

User interfaces need to be attractive and intuitive for non-specialists and usable from mobile devices and platforms commonly used in schools (such as chromebooks and tablets). Interfaces created for professionals do not necessarily work for non-specialists, because they tend to have the following characteristics: 1) offer too many options; 2) do not offer a clear path toward a learning outcome; 3) too slow,  unresponsive, or burdensome for the internet connections.  Effort should be spent on user interfaces for public audiences, and ideally, on creating introductory activities as preparation for more complicated tasks.

Surveying users to assess their needs and interests helps the content design process and continues to improve the quality of an experience for users when a program in running. User testing is a regular practice for many companies that deliver a product to the public and is a process that should be adapted within astronomy \gls{EPO} programs to ensure activities remain relevant and useable.

\subsubsection{Examples of online activities}
Several examples of existing and planned infrastructures illuminate avenues for online public engagement: below, we discuss Sloan Digital Sky Survey's (\gls{SDSS}) SkyServer, Zooniverse's \gls{Citizen Science}, \gls{NASA}'s Universe of Learning, and the \gls{EPO} program of \gls{LSST}.

For over 15 years, the \gls{SDSS} has made its vast database of imaging and spectroscopic data ($\sim$200 \gls{TB}) freely available to the world. The web-based \gls{SDSS} data browser, SkyServer\footnote{\url{http://skyserver.sdss.org}}, provides a public entry point for navigating the data online. The numerous and diverse query and analysis tools available through the SkyServer are designed to meet the needs of astronomers and non-professionals alike. The benefit to this design is that any interested student or member of the public has unrestricted access to research-grade inquiries and applications of the data.  However, the large number of available features and the technical jargon that accompany them often overwhelm non-experts, as well as professional astronomers who are external to the \gls{SDSS} collaboration.

In order to better support audiences who may be put off or overwhelmed by the professional-grade access points to the \gls{SDSS} database, the \gls{SDSS} Education and Public Outreach team developed activities with simplified query tools and smaller, curated datasets to facilitate activities for pre-college educators and students (e.g. \gls{SDSS} \textit{Voyages}\footnote{\url{http://voyages.sdss.org}}). For non-specialist audiences, these activities lower the barrier to accessing the same authentic data, while providing an introduction to concepts related to both astronomy and data structures.   For students and educators who may be interested in using the data for more advanced explorations, \gls{SDSS} Voyages provides a helpful stepping stone.  The next two sections of this chapter suggest avenues to promote this transition in other ongoing and planned astronomy projects and facilities.

%In response to this critical user feedback, SDSS decided to develop simplified tools and smaller, curated datasets to facilitate activities for pre-college educators and students (e.g. SDSS \textit{Voyages}\footnote{\url{http://voyages.sdss.org}}). This important transition marks a sea-change from creating EPO activities around existing research tools to the necessity of developing tools specific to  non-specialist audiences in order to make activities accessible to a broader range of people. The next two sections of this chapter suggest avenues to promote this transition in other ongoing and planned astronomy projects and facilities.

Citizen science represents an example of successful use of the modern age of web connectivity by directly engaging the public in scientific research. Online citizen science enables scientists to work with the general public to perform data-sorting and analysis tasks that are difficult or impossible to automate, or that would be insurmountable for a single person or for small groups of individuals to undertake \citep{2015ARA&A..53..247M}. Highly accessible citizen science activities can advance both science and learning in the era of large astronomical datasets. Moreover, most participants from the public claim that the main reason they participate is the contribution they are making to fundamental science research \citep{2017AAS...22941107C}. Through online citizen science portals such as the Zooniverse\footnote{\url{http://www.zooniverse.org}}  \citep{2011MNRAS.410..166L}, millions of volunteers have participated directly in this collaborative research experience, contributing to over 70 astronomy-based research papers. Another reason for the continued success of the Zooniverse platform in particular, is that it looks good and feels modern, even after a decade of activity. While professional astronomers are the \gls{PI}'s of citizen science projects, Zooniverse employs 13 developers, one designer, and two postdocs to lead the infrastructure development of the platform between the Adler and Oxford locations.
%2013arXiv1303.6886R,

Members of the Zooniverse team have furthered the project's educational impact by developing a college-level data science curriculum around their crowd-sourced data. The NSF-funded Improving Undergraduate \gls{STEM} Education (\gls{IUSE}) Project: ``Engaging Introductory Astronomy Students in Authentic Research through Citizen Science" (PI: L. Trouille) is a particularly successful example of scoping big-data astronomy for a college non-major audience. This innovative curriculum equips students with the essential tools to explore the intrinsic and environmental properties of 20,000 low-redshift \gls{SDSS} galaxies that have morphological classifications from Galaxy Zoo.  This project utilizes a curated dataset in Google Sheets and a simple, plug-in tool that enables intuitive data cropping and visualization. Instead of learning about galaxies and cosmology through traditional readings and lectures, students are challenged to discover key patterns and properties of the universe themselves, through first-hand explorations of authentic astronomical data. In the process, they gain skills in quantitative analysis, improve their overall data literacy, and practice science communication. The curriculum specifically provides an opportunity to discuss the complications and limitations of authentic data, and the challenges of framing a question that can be effectively tested with the data one has in hand. The project is a great case study of delivering specific, high-impact learning outcomes through an analysis of authentic data, without requiring students to navigate full-scale datasets or jargon-rich professional tools for visualization and analysis.

NASA's Universe of Learning\footnote{\url{https://www.universe-of-learning.org/}} offers a variety of individual online web pages that are well presented. A potential challenge for a typical user who finds one of these pages is knowing what to do next. Beyond exploring the beautiful multi-wavelength images space telescopes provide, there is not a clear path for a user to navigate toward specific learning outcomes or experiences.

%BN: Would discussing DES EPO fit in your narrative? We tried to be an unfunded precursor to the LSST effort (also showing what happens when you're not funded to do EPO).
% We mostly did the following:
% ... a decent web site
% ... social media (tried to be equitable and inclusive and diverse there in a few ways
% ... wrote summaries of papers for the public and reporters.
% ... wrote a white paper on our experiences.
% this may or may not be appropriate, just tossing it out there.

%AB: possibly.  DES EPO is an example of astronomer-led EPO effort. Was it successful in your eyes? In what ways could it have benefited from dedicated resources in the areas of expertise mentioned in \secref{eposkills}?

LSST’s \gls{EPO} program\footnote{https://www.lsst.org/about/epo} is unique among ground-based telescope projects: not only is it being constructed in tandem with the physical observatory itself, but the outreach program is funded at 2\% of the project cost. \gls{EPO} products will go live when the \gls{LSST} Survey begins in 2022. \gls{EPO} products were included from the beginning as part of the construction Project deliverables, because they faced similarly unique challenges as the data resulting from the survey itself. During its design phase, the \gls{EPO} team selected specific audiences and invested in user needs assessments to examine what these audiences want, and cannot find elsewhere. Some major findings include the necessity for mobile-friendly interfaces, a clear path toward learning goals, and educators needing no new \gls{software} to download in order to introduce classroom activities.  This has shaped the overall strategy for \gls{LSST} \gls{EPO} development and the skill sets needed on the \gls{EPO} Team, which is a small, interdisciplinary team of astronomers, writers, designers, educators, and developers. The mission of \gls{LSST} \gls{EPO} is ``to offer accessible and engaging online experiences that provide non-specialists access to, and context for, \gls{LSST} data so anyone can explore the Universe and be part of the discovery process.''

The operations website will feature news about \gls{LSST} discoveries, profiles of \gls{LSST} scientists and engineers and their work, and will be optimized for use on mobile devices. The \gls{EPO} team is also developing online, data-driven classroom investigation activities for students in advanced middle school through college. The topics cover commonly-taught principles in astronomy and physics, and each investigation is designed for use with Next Generation Science Standards (\gls{NGSS}) in the United States and the Curriculum Nacional in Chile. All investigations come with support and assessment materials for instructors and no special \gls{software} is needed to access the investigations, which will be available in English and Spanish. \gls{LSST} \gls{EPO} will maintain an easy-to-use gallery of high-quality multimedia visualizations that can be downloaded and integrated into exhibits and presentations. Finally, \gls{LSST} \gls{EPO} will provide support to researchers who create \gls{Citizen Science} projects using \gls{LSST} data, including a dedicated project-building tool on the Zooniverse platform. The infrastructure to host these activities is being built during construction and will take several years. Another critical task during construction is building prototypes and performing user testing, which has continually proven to improve the user experience and usability of interfaces.

A consistent theme that emerges when examining these examples is that well-defined learning outcomes for activities, curated access to authentic data, and simple, intuitive design are important to prepare for the \gls{EPO} response to the large data we will collect in the 2020s. The remaining sections identify areas of expertise \gls{EPO} teams can employ to achieve these outcomes.

\subsection{Bring expertise to astronomy education and outreach teams}\label{eposkills}

\nrec{EPO}{Manager, Educator}{Medium}{epo3}{Bring dedicated experts onto astronomy education and outreach teams}{To create the accessible online interfaces that maximize public impact in the next decade, we recommend supporting dedicated education and outreach teams that pair astronomers with technical and education specialists to increase relevance, adoptability, and accessibility of activities.}

The large-scale data challenges that face astronomy described in this paper also represent challenges and opportunities for formal education, public outreach, and science communication.  A natural instinct for astronomers may be to adapt their new computational experience to outreach efforts. This is a noble goal, but astronomers are not be expected to know effective practices around mobile-friendly development, intuitive user interfaces for the public, marketing through social media, or how to connect astronomy activities to formal education curriculum standards.  A team of \gls{EPO} experts can advise and assist with these areas, which are essential to build successful activities that are discoverable and adoptable.

We recommend astronomy organizations support creating \gls{EPO} teams with expertise in relevant areas. It is understood that to reach maximal impact of outreach activities, these individuals work with astronomers to combine astronomy and data science expertise with specific \gls{EPO} expertise and experience. This section describes options for areas of expertise and roles that can be brought on to achieve specific goals.

Educators in the \gls{US} are currently required to submit paperwork to demonstrate that they are teaching specific topics related to curriculum standards.  An \gls{EPO} {\bf education specialist or instructional designer} brings knowledge of relevant curriculum standards and rubrics (for example, the Next Generation Science Standards\footnote{NGSS: \url{https://www.nextgenscience.org/}}) and is able to connect astronomy activities to topics educators must cover. This is the most relevant for K-12 formal education in a traditional setting or homeschooling. An educational specialist can build professional development programs to increase confidence for bringing such activities into their classrooms if there is not an expert available to join in person.

An education specialist can also tap into educator networks to advertise existing programs and perform professional development. An example is the National Science Teachers Association (\gls{NSTA}) annual meeting and \gls{AAS}. An education specialist working with an astronomer can create curate datasets to achieve specific learning outcomes without overwhelming non-specialists \citep{Rebull18}.

An {\bf Information Officer or Communications Manager} can act as a primary contact for a facility and also set overall communication strategies and implementation plans. Topics covered in such strategies could include audiences, content priorities, communication channels, messaging, procedures, and more.

An {\bf Outreach Specialist} could serve a range of purposes depending on the needs of the group.  This could be a science writer, someone who responds to and directs questions received from audience groups, or contributes to social media presence.  or an astronomer trained in science communication. If this person has astronomy training, he/she could work with astronomical datasets to curate options for the public.

Social Media is becoming increasingly important as a source of news and information in society. Dedicating a full-time equivalent (or more) to the role of {\bf social media engagement specialist} increases awareness of \gls{EPO} activities and engages various audiences to participate with activities that exist.

Overall branding, the look and feel of online activities, and developing interesting graphics and images to support press releases or other activities are the role of a {\bf Graphic Designer}.

An {\bf evaluation specialist} informs methods for understanding the impact of programs on specific audience groups. The most benefit occurs when the method for evaluating the success of a program is built into the development of the program itself. Metrics could include and are not limited to web analytics, short or long surveys, interviews, login requests, focus groups, web submission forms, and social media interactions.

A {\bf web developer} considers the user interface and experience when visiting a site. Mobile-friendly accessibility is a requirement for non-specialists since most users of an online interface will discover the materials via social media and will access them from a mobile device, not a desktop  platform. In addition, the most common machines used by schools are chromebooks and potentially weak internet connections, which require lightweight design. Development needs to satisfy these requirements are best implemented by experts in the field.

A {\bf Software Architect} designs, deploys, and maintains production services for an online program. It is important to not overburden internet systems that can be common in classroom settings or non-urban areas.

A {\bf Project Manager} oversees the detailed budget, schedule, contracts, documentation, and reporting.  This role is important for programs being built during the construction of an astronomical facility.

\subsection{Fund dedicated astronomy education and outreach groups}\label{epogroups}

\nrec{EPO}{Agency}{Long}{epo2}{Fund dedicated or centralized astronomy education and outreach groups}{We recommend that funding agencies supporting the development and operation of large astronomical observing and data facilities fund professional education and outreach groups who can provide strategy, oversight, and best practices to maximize the impact of outreach efforts, and encourage \gls{EPO} efforts to be part of a project's mission.}

Having a dedicated individual or team to develop the \gls{EPO} program for a specific facility can improve efficiency, impact, and cost effectiveness. Strategic planning provides an opportunity to emphasize the identity of a particular large facility; to identify non-specialist audiences who could benefit the most from dedicated engagement; put into place best practices in outreach and communication programs; and complement the overall landscape of astronomy \gls{EPO} efforts. It is important that the \gls{EPO} professionals are employed directly at professional telescope facilities in order to emphasize the uniqueness of the program, build and maintain relationships with those doing the technical and scientific work, and help handle the astronomy-specific data products that currently require a reasonable level of understanding to interpret and use (see \secref{sec:data}).

A dedicated \gls{EPO} team also serves as a resource for enabling astronomers working with large datasets and data facilities to do more impactful and wide-reaching outreach. Groups that are specifically charged to do \gls{EPO} can improve the impact of the existing \gls{NSF} Broader Impacts investment by supporting astronomers to tap into existing programs. This improves discoverability of the \gls{EPO} work astronomers are doing increases the likelihood of achieving Broader Impact goals at both the individual and \gls{NSF} levels.

An \gls{EPO} team could provide any of the following benefits:
\begin{itemize}
\item Conducting science communication and media training sessions for astronomers doing these activities.
\item Providing introductions to various social media platforms that can be used for unique outreach experiences.
\item Marketing and promoting activities through established social media and common online training resources (e.g. Code Academy).
\item Creating or tapping into a centralized repository for people looking for resources
\item Creating opportunities for collaboration between astronomers and existing outreach infrastructure that will promote success and provide wide-reaching impact. Examples include {\em Journey Through the Universe} in Hawai’i or {\em AstroDay} in Chile, both led by Gemini \gls{EPO}.
\item Performing user needs assessments and user testing to improve the quality of existing activities and to develop new programs that meet the needs of specific audiences.
\item Evaluating and reporting on the impact of \gls{EPO} activities. Evaluation methods can and should be built into program design.
\item Providing guidance for astronomers when developing science drivers and use cases for educational materials and public interfaces related to their research expertise.
\item Broadening participation to non-traditional audience groups.
\end{itemize}



%LSST’s focus group testing / evaluation
%A. Colantonio, S. Galano, S. Leccia, E. Puddu, and I. Testa, Design and development of a learning progression about stellar structure and evolution, Phys. Rev. Phys. Educ. Res. 14, 010143 (2018).; D. F. Barringer, J. D. Plummer, J. Kregenow, and C. Palma, Gamified approach to teaching introductory astronomy online, Phys. Rev. Phys. Educ. Res. 14, 010140 (2018).

%NSTA, Nsta position statement: Professional development in science education (2006) - \url{https://www.nsta.org/about/positions/profdev.aspx}

%National Science Board STEM Education Recommendations to the Obama Administration \url{https://www.nsf.gov/nsb/publications/2009/01_10_stem_rec_obama.pdf}

The timing for building expert \gls{EPO} teams should occur during the construction of a new facility and be included as part of the project's mission.  Starting early affords time to implement appropriate strategy and infrastructure.  Educational materials, supplemental professional development materials, striking visualizations and images and communications strategies should be ready at the start of a project to maximize the public impact of the facility.



In this chapter, we discussed recommendations and effective practices that can be employed to maximize the impact of large astronomy facilities and data centers in the next decade. We prefaced the need for creating accessible online astronomy activities for the public and identified a range of skills needed to create such activities. Finally, we established the benefits of resourcing dedicated \gls{EPO} groups from the earliest stages of astronomy facility planning and even including \gls{EPO} as part of the mission of projects.

These recommendations are based on two main things: trends seen elsewhere on the web that successfully respond to this new era of technology and social interactions on the web, and case studies within astronomy that demonstrate appropriate avenues for increasing engagement and accessibility through online activities.

Note: This chapter is the basis for an Astro2020 Decadal Survey \gls{APC} white paper which will go into detail on resourcing and prioritizing recommendations. If you are interested in commenting or constributing, please contact Amanda E. Bauer <abauer@lsst.org>.




==> old_text/intro.tex <==
\section{Introduction\Contact{William O'Mullane}}\label{sec:intro}

\Contributors{William O'Mullane <\mail{womullan@lsst.org}>, Ting Li <\mail{tingli@fnal.gov}>}
\bigskip

%{\color{red} If you spot editorial inconsistencies please note them here \url{https://docs.google.com/document/d/1aXjB_TZ6aJN6ryXF82O8gBCsk6EeJ-4vA6fhg7Aci3A/edit?usp=sharing} comments on content can go directly to overleaf or slack}

In the Petabyte era the lines between \gls{software}, technology and science are blurred - the chance to do science with petabytes without major infrastructure is pretty slim. Therefore the importance of technology in science exploitation becomes ever more important, which also implies we pick up the pace in training the workforce and in the areas of education and public outreach.

The Kavli foundation sponsored a series of workshops on the theme \emph{Petabytes to Science}\footnote{\url{https://petabytestoscience.github.io/}}, the second of which was held 12$^{th}$ to 14$^{th}$ of February 2019 in Las Vegas.
The aim of the this second workshop was to formulate potential \gls{APC} white papers. To facilitate this we
 discussed important trends,  technologies, approaches to workforce management, education and public outreach.
We took a holistic approach and built a single document encompassing several broad categories, namely:
\begin{itemize}
	\item Science drivers (\secref{sec:science}) - which science cases need new techniques and approaches?
	\item Data Management (\secref{sec:data}) - what data management challenges does this present?
	\item Software (\secref{sec:software}) - how should \gls{software} be developed to meet those challenges?
	\item Technology and Infrastructure (\secref{sec:tech}) - what technologies and infrastructure is needed to under pin the services?
	\item Workforce and Inclusion (\secref{sec:iwft}) - what training should we do to prepare ? How can we improve and diversify the workforce?
	\item Education and Public Outreach (\secref{sec:epo}) - through \gls{EPO} can we increase awareness of the public about astronomy and ensure future finding streams? What are the challenges and opportunities for EPO?

\end{itemize}

From each of the sections a number of recommendations were identified, these are summarized in \secref{sec:recs}.
For each recommendation we suggest the audiences they are useful to and the time period in which they should be executed (this may be seen as a sort of priority). The time periods or terms are short term (1-3 years), medium term (3-5 years) and long term (5-10 years).

The intention is to extract some decadal survey \gls{APC} papers from these ideas.
If you are interested in contributing to or endorsing
\href{https://tinyurl.com/y2ksemp2}{white papers on these topics sign up here}\footnote{\url{https://tinyurl.com/y2ksemp2}}  or contact the authors listed in this document -- names followed by an email address are the leads of each chapter.


\noindent\textbf{Note:} This document is a collection of ideas and a record from a workshop  - it is not a polished document.  We
have made some effort to not have repetitions between chapters however we do not guarantee a pleasant coherent read.


==> old_text/iwft.tex <==
\section{Workforce \& Career Development \Contact{Dara Norman}}
\Contributors{Dara Norman <\mail{dnorman@noao.edu}>, Kelle Cruz, Vandana Desai, Britt Lundgren, Eric Bellm, Frossie Economou, Arfon Smith, Amanda Bauer, Brian Nord, Chad Schafer, Gautham Narayan, Ting Li, Erik Tollerud}
\label{sec:iwft}

\bigskip
\input{caveat}

%\subsection{Draft Recommendations}
%\begin{itemize}
%\item \rec{wc4}{Coding and data skills into existing courses}{Professional Societies, Departments and individuals must encourage educational programs to incorporate coding and data skills into their existing courses and programs.}
%\item \rec{wc5}{Career paths}{Agencies should continue to support (and resource) data centers and departments to develop career paths around software \& big data science.}
%\item \rec{wc6}{Recommendations to journals}{Journals should adopt software refereeing and clarity on guidelines for citing technical contributions.}
%\end{itemize}
\subsection{The growing importance of a tech-savvy workforce of astronomers}
In the rapidly approaching era of large surveys, experiments, and datasets, we will only reach our scientific goals if we train and retain highly capable scientists, who are also engaged with technological advances in computing.
%BN: Put EXCERPT A here (see below)
With the goal of advancing scientific discovery through the collection and analysis of data, we must commit and dedicate resources to building both the skills and competencies of this workforce.
%BN: (replacing previous sentence)
% A workforce that is skilled and competent in the collection and analysis of scientific data is a critical requirement for distilling discoveries from big data.
%BN: We must dedicate resources to developing and training this workforce.
%This includes those in the workforce that will be using data to advance science as well as, those  supporting the infrastructure that make those discoveries possible.
%BN: (replacing previous sentence)
 We define the workforce as those who derive science from the data, as well as those who build the infrastructure to collect and prepare the data for discovery analyses; one cannot happen without the other.
The areas and skill sets in which our teams need training are \gls{software} carpentry, algorithms, statistics, the use of software tools and user services; and \gls{software} engineering effective practices, data management and access (for support staff).
In addition, all members of the workforce, including those who provide infrastructure, will require professional development opportunities and support for their career advancement allows them to remain as productive and respected members of the field.

In this chapter we discuss the activities needed to build, support, and advance the scientific workforce that will take the petabytes of data collected to scientific discoveries over the next decade. In particular, \secref{sec:iwft:demographics} discusses the current demographics of the data science support mission while (\secref{sec:iwft:software}) exemplifies the scope of training that is needed to build this workforce. \secref{sec:iwft:datascience} focuses on training for researchers who are more accurately described as ``users.''  In \secref{sec:iwft:careers}, we discuss modern challenges for these career paths, as well as how to address them. Finally, in \secref{sec:iwft:credit}, we identify  metrics that we should be using for training in career development and for reviews in career advancement.


\subsection{Demographics - who is this workforce and where are they now\label{sec:iwft:demographics}}
Data support roles are spread throughout the astronomy and astrophysics (hereafter, ``astronomy'') scientific community, and encompass people with a variety of job types and descriptions at levels from post-baccalaureate to PhD.
% A range of experience with either topics of astronomy or computing also differentiate roles.
A range of experience with either topics of astronomy or computing also differentiate roles.
This range of data support positions requires a diversity of opportunities for training to work at the various levels. In addition, different career development and advancement suited to those career tracks is also required.
For example, positions for those with PhDs are significantly different from those that require only a post-bac degree, and thus the metrics used to support and determine career advancement must also be different.  It has only recently been recognized that this role should be trained for and tracked independently of scientific interests and other professional duties.
Consequently, the community has not adequately tracked the quantity and demographics of astronomy researchers currently engaged in science data support roles.

Instead of quoting statistics here, we present exemplar descriptions of current job titles and roles.
Many of the people engaged in science data support hold PhDs in astronomy, astrophysics or physics.  These researchers may be employed at colleges, universities, data centers or observatories, national laboratories. They may hold a leveled academic title (e.g. Professor, Astronomer, Scientist, etc.), as well as an additional functional job position in centers or programs with names ``Data Science Mission Office,'' ``Community Science and Data Center,'' ``Infrared Processing and Analysis Center.''
%Meeting career milestones to move up the ladder in these academic titles (i.e. assistant, associate, full, etc.) currently often only include the same metrics as for other faculty and staff (e.g. numbers of published papers, h-value, etc.)
% BN (replacing previous sentence)
 Despite the distinct nature of the work for scientists who hold these multiple roles/titles, the same metrics (e.g. numbers of published papers, h-value, etc.) for career advancement through titled positions (i.e. assistant, associate, full, etc.) are used for them as for faculty with more typical duties and responsibilities.
More discussion is in \secref{sec:iwft:careers}.

There are also many other science data support roles, in which staff have degrees at the BS, MS, or PhD level with position titles like ``research and instrument associate,'' ``research and instrument scientist,'' ``mission systems scientist,'' ``archive scientist.'' These staff are often responsible for coding and database support.
Below, we discuss the resources and cultural changes needed to support the career trajectories of this workforce, to slow the threat of ``brain drain'' from the field, and to develop a workforce that can thrive in academia, industry, or government lab positions.
%DO we need more about what these duties entail or no?

\subsection{Training to contribute to \gls{software} development: Building the next generation\label{sec:iwft:software}}
%\subsubsection{Education}
%[From Gautham - Likely to move to EPO or workforce development]

Astronomers have a long history of developing useful \gls{software}, but \gls{software} development itself has not been considered a core component of the astronomy training curriculum. The expectation of petascale datasets in the 2020's provides a strong motivation to increase familiarity with effective practices in \gls{software} development, as well as with existing frameworks that are widely used in the commercial sector. This cultural change will lead to better \gls{software} in astronomy and more innovative scientific discovery. It will also provide astronomers with invaluable training that will increase their familiarity with (and marketability to) work in industry.

Currently, effective practices include using \gls{version control} (e.g. GitHub), maintaining documentation and unit tests with code, and employing continuous integration methodologies, in which code is built and executed in shared repositories, allowing teams to identify issues early. Analysis in the 2020s will involve many pieces of \gls{software} that are integrated into complex pipelines, processing ever-larger volumes of data. Astronomical projects are now comparable in scale to large industrial \gls{software} development projects. Consequently, the gap between these effective practices and the modern cultural norm in astronomy and astrophysics must be reduced as the field transitions to increasingly large collaborations.

The increasingly critical role of \gls{software} development in astronomy clearly indicates it is crucial that \gls{software} development become part of the core graduate curriculum alongside typical coursework, like mathematics and observing techniques. Such coursework will also help reduce the disparity between students from diverse backgrounds, some of whom may never have been exposed to \gls{software} development, or even coding, as undergraduates. This course material complements, but is distinct from, training in data science and scientific computing techniques, which are increasingly being incorporated into Astronomy coursework. Developing the course material for data science work is likely beyond the scope of most departments, but vital steps have already been taken by several groups. Notably, the \gls{LSST} Data Science Fellowship Program has already developed materials to expose students to best practices for \gls{software} development. Curating these materials, and augmenting them with information for distribution on widely-used platforms will reduce the barrier to adopting such coursework or integrating it into existing classes.
%We also recommend summer schools and workshops targeted at mid-career and senior astronomers, to ensure that their skills are also honed. Astronomy can benefit from tapping into the large pool of researchers who are now actively employed in software development and data science, and encouraging these scientists who have crossed over to industry to expose those within the academe to the state-of-the-art. %DJN This is covered in the next section, but perhaps should put a aomment about that.

Besides developing course material, there are several other challenges to supporting scientific \gls{software} training in a university setting. Another challenge is the lack of access to state-of-the-art technologies. Because the landscape of coding and \gls{software} development changes rapidly as coding languages come and go, workflow best practices continually evolve, and new platforms emerge and gain wide acceptance. For principal investigators and project managers to make informed decisions and guide their teams, there must be opportunities for them to stay abreast of these developments and to evaluate their utility even if they are not the ones actually using the various tools.

Yet another challenge resides in the structure and processes of university departments. Many computer science departments do not teach the programming skills necessary for scientists.
% (might want to soften this generalization... some are.)
%Even if they did, departments are unlikely to want to send their majors to take classes in other departments.
%and many Astronomy departments are not resourced well enough to develop new courses themselves, much less teach them.
Current  faculty, especially at smaller, under-resourced schools, do not have the resources to develop these.
Thus, the burden of developing more appropriate materials is fractured and currently falls upon individual instructors. The field needs dedicated staffing to develop curriculum materials for computational training. A fundamental barrier to the development of reliable, curated, and widely shared \gls{software} in astronomy is the lack of incentives for this work and the dominance of the ``publish or perish'' mentality. Changing this cultural norm requires that our community incentivize --- both within scientific projects and across the field at the employment level --- work in developing good \gls{software} and in educating people to build good \gls{software}.
%Recognizing such work in assessing service and research, and valuing well-written and -documented \gls{software} that is widely used for scientific work, rather than only immediate personal results is a vital step in changing this culture and in preparing the field for the \gls{software} challenges that will be posed by massive projects in the 2020s.
% BN (replacing previous sentence)We need to make t
Two key updates must be made to our community's value structure to change cultural norms and prepare for the software challenges of projects in the 2020's: 1) software development work should be a part of assessments in service and research; 2) software that is widely used for scientific work should be well-written and -documented.
A full solution cannot be realized through universities alone, and partnerships with data centers, observatories, national labs, and professional societies are crucial.

The clear successes and popularity of the existing training programs, which grew organically out of the community, attest to the need for additional and more advanced training resources. While there are several successful programs that address some of these concerns, they are insufficient to meet the needs of the larger community.  For example, the Software Carpentry curriculum (\url{https://software-carpentry.org/lessons/}) is limited to the very basics of \gls{version control} and collaborative \gls{software} development but does not cover topics, like performance optimization, continuous integration and testing, and documentation. Furthermore, most of these workshops are targeted to senior graduate students, with a few targeting very early-career scientists, and they are not designed to meet the needs or concerns of mid-career scientists and managers. Thus, these programs are currently limited to a very small portion of the community and are currently unable to  provide the needed training to people in multiple sectors of our community who need and want these opportunities.
%Events organized by the astronomy community such as “hack” events (2018PNAS..115.8872H), the Python in Astronomy conference.   --- this fragment was here but not sure why...

Staff at Data Centers may themselves currently lack up-to-date data science skills and  knowledge. Funding to support career development for current staff and to provide resources for centers to hire staff that have data science expertise is critical to building workforce capacity in the 2020s.

Fundamental coding and \gls{software} development skills are becoming increasingly necessary for success in every aspect of Astronomy. However, acquiring professional training in these skills is rare and inaccessible or impractical for many members of our community. Students and professionals alike have been expected to learn these skills on their own, outside of their formal classroom curriculum or work duties. Despite the recognized importance of these skills, there is little opportunity to learn and build them --- even for interested researchers. %and would like to obtain them, there is no room in their schedule for this learning.
To have a workforce capable of taking advantage of the computational resources and data coming in the next decade, we must find and support ways to make coding and \gls{software} development training widely accessible to community members at all levels.

 \nrec{Workforce}{Agency }{Long} {wc3}{Programs to cultivate the next generation}{Agencies should fund more and large-scale programs that cultivate the next generation of researchers versed in both astrophysics and data science, similar to smaller and over-subscribed programs like Software and Data Carpentry, \gls{LSSTC} Data Science Fellowship/ La Serena Data School for Science, Penn State Summer School in Statistics for Astronomers.}

 \nrec{Workforce}{Agency }{Short} {wc4}{Support to produce training materials}{Provide funding to data and computational centers to produce modular and re-usable training resources to the community. These resources should be designed to be used by individuals, integrated into formal classes, and used as part of professional development training.}

 \nrec{Workforce}{Agency }{Long} {wc5}{Long-term curation of materials}{Funding must be provided to host and support educational materials in a long-term, stable, scalable place. Provides stability and improves discoverability if materials can live in a centralized location.}

 \nrec{Workforce}{Agency }{Medium} {wcfundpartner}{Funding for innovative partnerships}{Incentives should be provided to launch opportunities to harness partnerships between data centers, universities and industry through funding. For example, support for sabbatical programs at the data centers where teaching faculty can learn skills, develop educational materials for community use, and bring back to their home institutions.}

 \nrec{Workforce}{Astronomer, Educator, University }{Medium} {wc6}{Software training as part of science curriculum}{Individuals, departments, and professional societies should encourage educational programs to incorporate \gls{software} training skills into their existing courses and programs.}
%Encourage departments to offer regular trainings.

%Current small scale examples of this kind of training are:

%\begin{itemize}
%\item Software Carpentry
%\item Python in Astronomy
%\item AstroHackWeek
%\item DotAstronomy
%\item Astropy Tutorials
%\end{itemize}



%One option is for the data and science centers to consider educators part of the user community and develop educational materials alongside documentation.

%Below we outline recommendations for how various actors could contribute towards fostering a culture within the Astronomical community of life-long learning on computation and software development topics.


\subsection{Training to take advantage of big data for research: Bytes to Science\label{sec:iwft:datascience}}
Astronomers who came of age before the era of Big Data require training to take advantage of astronomical “Big Data” in the 2020s. They also need these skills to mentor students, who are simultaneously learning both astrophysics and the uses of data for research. It is crucial that access to this training be made widely available to professionals who come from a variety of science backgrounds and are based at a broad range of institutions (e.g. universities, data centers, etc.). This is especially important, considering these professionals will be cultivating their students and the next generation of scientists, as well as making decisions about which technologies to invest in. If access to advancing data skills remains difficult to obtain, we will fail to build a diverse workforce equipped to answer the most pressing questions in astronomical research. Data Centers could play an important role in providing this training.

New, freely accessible open source code and Jupyter frameworks like SciServer.org and \gls{NOAO} Data Lab enable anyone with a web browser to quickly and easily analyze vast stores of professional astronomy datasets via web-based notebooks.  These cloud-based platforms can democratize educational access by providing a scale of computing power and data storage that was previously reserved for students and faculty at well-resourced research institutions, where high-performance computing access and support are abundant.  A small number of astronomers in higher education are already developing instructional activities for these platforms. These instructional materials train students and other users to explore and analyze large professional astronomy datasets with ease and to equip users with the computational foundation needed to pursue advanced independent research projects.

Jupyter notebooks in particular hold enormous potential for training the current and next generation of astronomy professionals. However, currently, the development of standardized curricular activities is performed in an entirely ad-hoc manner.
Limited resources (funding and time) lead to very little deliberate coordination amongst various astronomy faculty who produce such materials, and these products are not sufficiently discoverable (e.g. accessible through a common repository).

%There needs to be a recommendation about this idea of better supporting the technology that we are building curriculum on...Is this a funding issue and/or an ability to gain scope for the data centers?  Is it exclusively something that can be solved by funding agencies?
%However maybe it is a recommendation in another chapter like infrastructure?

The establishment of Community Science Centers hosted by Data Centers (like \gls{NOAO})  can be a hub (clearing house) to bring information to the community about opportunities for the kind of resources and training that allow a broad group of researchers to go from petabytes to publications.


% Too much in the weeds here:  and task these staff with training responsibilities. These tasks could include responding to Help Desk questions, moderating online forums, hosting webinars and workshops, creating video tutorials, and writing sample code (e.g. jupyter notebooks).

%In order for students to hit the ground running in their graduate careers, a modern undergraduate astronomy education should include computational methods as an integral part of the experimental and theoretical core curriculum.  Teaching these skills with the use of authentic scientific data can further enhance the learning process and have positive effects on student interest and persistence.

%This might fit better in section 8.3
%Training Students


In order to provide the most useful training, data centers need a clear view of user needs. This information is provided by advisory committees, like ``User Panels.'' However, these panels are traditionally populated by astronomers based at R1 institutions and other data centers. Data Centers should ensure that their User Panels include representatives from small and under-resourced institutions; this will provide a clearer picture of the unique training needs and challenges that must be addressed for these researchers.  In addition community surveys that reach astronomers who do not currently use data centers should be undertaken to better understand what barriers exist.

 \nrec{Workforce}{Agency }{Short} {wc1}{Training activities and materials}{Agencies must ensure that big data science training activities and materials for PROFESSIONALS (as well as students) are included as part of the federally funded data center’s mission and deliverables.}
 \nrec{Workforce}{Agency }{Medium} {wc2}{Change advisory board representation}{Federally (and privately?) funded science centers should include representatives from small and under-resourced institutions to provide a broad and clear picture of need in the community.  The collection of information, perhaps through surveys, to better understand the barriers to access that exist for astronomers at these institutions should be undertaken by data centers and others.}


\subsection{Identifying career paths around scientific \gls{software} development \& big data science\label{sec:iwft:careers}}
The key skills necessary for data-intensive scientific research are also highly valued in industry, government, and media/communication sectors. Astronomy training can serve as a stepping stone to fulfilling careers in a wide variety of fields, and astronomers should support and encourage those who transition to jobs in non-academic science, because ties with industry can strengthen and leverage our partnership opportunities. However, we need informed people on both sides: in many cases, challenging and uncertain career paths in astronomy push the best and brightest towards careers where their contributions are more readily appreciated. This ``brain drain'' siphons away the very researchers most needed to tackle the most pressing science questions of the 2020s.

\subsubsection{Universities}
In the university context, tenure-track faculty positions remain the gold standard for stability, compensation, and prestige.  However, despite the  fundamental role of \gls{software} in scientific discovery, it remains difficult to receive credit towards tenure and promotion for developing \gls{software} and services.  \secref{sec:iwft:credit} offers more specific recommendations for improving recognition for these contributions.

Even with appropriate credit for \gls{software} contributions, faculty positions will continue to carry expectations of leadership, grant-writing, teaching, mentorship, and service, as is appropriate.  Furthermore, driven by ongoing changes in the landscape of higher education, tenure-track hiring continues to flatten.  To benefit from the opportunities of large datasets, universities also need the ability to support and retain technically capable faculty and staff, who have expertise and a longevity that typically cannot be matched by graduate students or postdocs.  These “Research Software Engineers” (\cite{rse}) would provide a technical core for data-intensive research groups, just as opto-mechanical and electrical engineers are vital to the success of instrumentation labs.

Stable funding is the largest need for the success of staff Research Software Engineers \citep{geiger_2018}. A patchwork of 2-3-year soft-money grants is insufficient to retain highly-capable professionals, especially when industry salaries are significantly higher. Universities should explore means of providing internal support for data science staff, perhaps sharing capacity between academic groups or departments.
Long-term vision and leadership in the field are needed to recognize and measure relevant metrics and make them part of advancement/career ladders.


 \nrec{Workforce}{Manager }{Short} {wcA}{Recognize  software as part of the career path}{Software should be recognized in hiring and career development as a core product of modern astronomical research. Software outputs should be considered in all aspects of academic performance appraisals, career applications, and promotion and tenure review cases. }
  \nrec{Workforce}{University }{Medium} {wcB}{Partnerships to support data science staff}{Universities should explore means of providing support for data-science faculty and staff, perhaps sharing capacity between academic groups or departments internally or partnerships outside the university.}
  \nrec{Workforce}{Agency }{Medium} {wcFund}{Support long-term technical capacity}{Funding agencies should explore longer-term grants aimed at building and supporting professional (non-student) data science capacity.}


\subsection{Elevating the role of software as a product of the research enterprise}

%Software is a critical part of modern research and yet there is generally poor support across the scholarly ecosystem for its acknowledgment and citation, and in turn, for measuring its impact. The majority of academic fields rely on a one-dimensional credit model whereby academic articles (and their associated citations) are the dominant factor in the success of a researcher’s career.  %CITATION NEEDED?

%In the petabyte era of astronomical science, making it possible to easily cite  software and measure its impact is going to be critical for maximizing the scientific return of these large datasets and retaining those individuals who specialize in developing the tools to turn them into publications.

%Evolving beyond the one-dimensional credit model requires overcoming several key challenges including the current scholarly ecosystem and scientific culture issues.  Career paths for staff, including scientific staff,  in these technical roles need to have clearly defined metrics and requirements that take into account how they are required to spend their time in support of the scientific enterprise.

%\begin{itemize}
 %   \item{\textbf{The scholarly ecosystem}:
    % "is not under our control" this is not entirely true and the argument needs to be revised and clarified.  Publications like ApJ and  AJ} are run by  AAS} societies which are answerable to their boards which are elected by the membership (researchers who publish in them).  Thus while it may be difficult to change the system, there are mechanisms in place and this is as much under "our" control as anything is. As is this paragraph is defeatist and comes off as unproductive.
    %Even if we wanted to evolve the existing model, we publish our work in journals, many of which are not controlled by the researchers who publish in them. Any change we might want to see, such as the ability to cite  software natively in papers (\cite{Smith2016}) requires changes to systems (journal publishing systems, indexers) not owned by us. We note that in recent years, substantial progress has been made in astronomy and astrophysics on these topics including changes in editorial policies by  AAS} publishing (\cite{aassoftware}), and partnerships with journals specializing in  software review (\cite{Vishniac_2018}).

The ecosystem around the publishing of scholarly work has not been set up to properly account for contributions to scientific discoveries made through tools, services and other infrastructure.  Changes for the modern way in which science is done need to be made.  Publications, like ApJ and  AJ , are run by the  AAS , a professional society, and are answerable to their boards that are elected by and comprise the membership of professional researchers, who also publish in them. Therefore, it is important to educate the larger community on changes that need to be made to support modern recognition standards for  software services and then advocate for these changes with professional societies.

Social and cultural issues within the field also must be changed to normalize the appropriate acknowledgment of those who write  software and support other science infrastructure tools.
We need academics in positions of power (e.g. on promotion and tenure review committees, recruitment teams, grant review panels) to value  software as an important product of research. Although change takes time, it is important that we begin making those changes with concrete and practical suggestions that can be incrementally introduced into accepted procedures and communal norms. These suggestions include the identification of metrics that support proper assessment of the impact of  software on achieving scientific results.  In recent years, substantial improvements to enable the citation of  software and tracking of these citations has been made in astronomy and astrophysics.
%\end{itemize 

%

\subsubsection{Measuring\/citing the impact of software

One key factor for improving the recognition of software within academia is to enable native software citation, that is, make it possible and required for authors to cite the software packages they have used in the process of carrying out their research, and to then count these citations in tools such as the Astrophysics Data System ( ADS ). Enabling software citation is both a technical challenge and a cultural one: recommendations for what software should be cited and when to cite it have been explored in community-wide effort at  FORCE11  \citep{Smith2016}, and follow-on efforts are exploring some of the more technical aspects of how to implement these recommendations (\cite{force11softwareimplentation}).

Within astronomy and astrophysics, the Asclepias project \footnote{\url{http://adsabs.github.io/blog/asclepias}  --- a collaboration between  AAS publishing,  ADS, and the Zenodo data archive  \citep{henneken_edwin_2017_1011088} --- is working to enable first-class support for  software citation in  AAS journals as well as support for indexing (counting) these citations within  ADS. While this project is currently scoped to  AAS  journals only, the changes being made to support the citation and indexing of  software serve as an example for other journals to follow suit.

\subsubsection{Strategies for elevating the role of software}

Part of the challenge of elevating the role of  software within academia is to find actionable changes that improve the career prospects of those individuals writing research  software. In this section, we outline a number of possible approaches.

\textbf{Software papers}: One approach gaining traction across a number of research disciplines is to allow papers about  software to be published in ``conventional'' journals alongside other research papers, thereby making  software more visible to the academic community, and giving  software engineers a citable ``creditable'' entity (a paper) to include on their resume. Examples of journals within astronomy that demonstrate a willingness to follow this approach include PASP\footnote{\url{https://iopscience.iop.org/journal/1538-3873}  and  AAS  publishing, which recently changed its editorial policies to explicitly allow  software papers in their publications \citep{aassoftware}. More recently  AAS  publishing has announced a partnership with another journal specializing in  software review \citep{Vishniac_2018}.

\textbf{Enabling support for  software citation and indexing}: Another key factor in raising the visibility of research  software is to enable  software citation, count these citations, and then make these metrics visible to the world. As part of the work of the Asclepias project,  software citations are not only being counted in the astronomical literature, they are also being made visible on the  ADS  website next to the paper record on  ADS .

\textbf{Inform and educate the community about  software contributions}: Organizations play a critical role in improving the career prospects of those writing research  software as they are responsible for hiring these individuals, evaluating their performance, and making decisions about possible promotions/career advancement. One immediately actionable approach is to encourage prospective employees and current staff to list  software they have developed on their resumes and performance appraisals. This would allow review committees to include  software as part of their evaluations.

\textbf{Community prizes}:  AAS  has a collection of prizes for scientific merit, instrumentation, education, and service to the field. As it is an important part of scientific discovery,  software contributions that have had a lasting positive impact on the field, should also be recognized with a new dedicated prize and/or as a recognized example of merit within these other prize categories.

\textbf{Grants}: The amount of research funding secured is an established metric for evaluating an individual. As recommended in software, allowing existing funding streams to be utilized for  software development provides a simple mechanism for funding research  software, but also signaling community recognition for the impact and relevance of the individual writing this  software. Furthermore, widespread availability of grant funding in support of  software development would provide a strong incentive for universities to hire technical astronomers into tenure track positions.

 \nrec{Workforce}{Astronomer }{Short} {wc8}{Adopt best practices for  software citation}{Journals and reviewers should adopt best practices for assuring that  software and other science support infrastructure is properly referenced and cited in articles.  Referees and other reviewers should be trained to recognize when such acknowledgement is necessary and ask authors to provide that information.}
 \nrec{Workforce}{Manager }{Long} {wc9}{Adopt promotion metrics that acknowledge  software and other science support}{Departments and other members of the community should adopt and use suggested metrics for promotion and tenure reviews of those scientists whose work and contributions involve  software and science infrastructure.}
 \nrec{Workforce}{Agency }{Short} {wc10}{Community prizes for  software contributions}{Professional astronomy societies should create dedicated  prizes and allow for software contributions to be recognized as a criteria of merit within existing prizes. }


\bigskip

\end{document}


\bigskip








==> old_text/science-v2.tex <==
\section{Scientific Context and Drivers}\label{sec:science}


%\noindent\Contact{}

\noindent\Contributors{Adam Bolton <\mail{bolton@noao.edu}>, Eric Bellm, Alex Drlica-Wagner, Ting Li, Raffaella Margutti, Gautham Narayan, Meg Schwamb}
\bigskip

\input{caveat}

The last two decades have seen a significant increase in the prominence of data-intensive, survey-scale astronomy. Surveys such as \gls{SDSS}, \gls{DES}, \gls{Pan-STARRS}, and \gls{ZTF} have pioneered these modes. Even more ambitious projects such as \gls{DESI}, \gls{LSST}, \gls{WFIRST}, and \gls{SKA} are rapidly approaching, bringing new opportunities and challenges for petascale astronomical science.

From an experimental design perspective, the development of large survey projects and facilities has been driven by fundamental scientific questions about the Solar System, our Milky Way and its stellar populations and satellites, the evolution of galaxies and quasars, and the nature of dark matter and dark energy. These questions have in common the need to obtain significant statistics over large population samples or volumes, or alternatively, to realize significant probabilities for the discovery of rare objects or events.

Big surveys naturally lead to big datasets. These big datasets in turn bring qualitatively new challenges in data management, computing, \gls{software}, and professional development that must be tackled to realize the scientific promise of the surveys themselves.

Big datasets from big surveys also open up diverse opportunities for \textit{data-driven science}: research and discovery programs defined entirely on the basis of available datasets, not on the basis of collecting new data. This approach is especially empowering of exploratory science, as described in the series of Astro2020 white papers by \citet{Fabbiano_wp_103,Fabbiano_wp_102,Fabbiano_wp_101,Fabbiano_wp_100,Fabbiano_wp_98,Fabbiano_wp_99}. Data-driven research can multiply the scientific impact of a survey, and can be especially effective for broadening participation in forefront astronomical research beyond those groups with the greatest access to resources. Data-driven science with large surveys calls on many of the same data-intensive methods as are required for ``primary'' survey science, while also presenting new challenges and requirements such as public data release and broad data accessibility.

In the following subsections, we outline some  current scientific opportunities, and their associated data-intensive challenges, across a broad range of astrophysics and cosmology drawn from science white papers submitted to the Astro2020 Decadal Survey. In the subsequent chapters of this report, we address the crosscutting technology, methods, and professional considerations that will support success in these scientific areas in the next decade.

\subsection{Planetary Systems; Star and Planet Formation}

LSST will conduct a 10-year survey across the southern sky, revisiting the same locations approximately every three days. This time-resolved dataset will detect both transient objects in the fixed sky and moving objects in the Solar System. \citet{Chanover_wp_378} describe the promise of \gls{LSST} for the discovery of \textit{dynamic} Solar System phenomena such as active asteroids and small-body collisions. To yield their scientific potential, these objects require rapid detection, alert, and follow-up observation. This implies the need for a coordinated real-time \gls{software} infrastructure beyond the scope of \gls{LSST} operations deliverables. Similarly, \citet{Holler_wp_79} describe the Solar System science potential of \gls{WFIRST}, which will require the deployment of robust moving-object detection algorithms within the \gls{WFIRST} data management framework.

A core goal of the \gls{WFIRST} mission is to conduct a microlensing census of extrasolar planets. \citet{Yee_wp_425} and \citet{Gaudi_wp_235} describe both core and ancillary science potential of this aspect of \gls{WFIRST}, which highlights the algorithmic and software-systems engineering challenge of addressing diverse microlensing applications within a petascale dataset with quality comparable to space-based telescopes.

\citet{Ford_wp_517} discuss the essential role of advanced statistical and machine-learning methodologies for optimal extraction of Doppler signatures of extrasolar planets with high-resolution spectroscopy in the coming decade. As the experimental forefront approaches the 10 cm\,s$^{-1}$ precision necessary to detect true Earth analogs around Sun-like stars, new statistics and algorithms become ever more crucial.

\subsection{Stars and Stellar Evolution; Resolved Stellar Populations}

\citet{Pevtsov_wp_212} highlight the potential scientific return for stellar astrophysics from digitizing historical astronomy data and making it available in accessible forms within modern data-management systems.

\citet{Dey_wp_541} and \citet{Kollmeier_wp_557} describe the potential for data-mining within large spectroscopic survey datasets (e.g. \gls{SDSS}, \gls{DESI}) to discover primordial Population III stars as well as new, rare, and unexpected stellar types.

Several Astro2020 white papers highlight the scientific potential that arises from combining multiple large-scale resolved stellar datasets. Asteroseismology results can be sharpened through the combination of time-series data from \gls{TESS}, \gls{PLATO}, and \gls{WFIRST} with stellar spectroscopic parameters measured by SDSS-V, \gls{MSE}, and other surveys \citep{Huber_wp_540}. Our knowledge of the structure, formation, stellar populations, and cosmological context of the Milky Way will be maximized through the combination of photometry, astrometry, and spectroscopy from multiple survey missions \citep{Sanderson_wp_387,Williams_wp_337}. Joint time-resolved analysis of photometric, astrometric, and spectroscopic survey data will also enable diverse astrophysical applications of stellar multiplicity \citep{Rix_wp_119}. For all these scientific goals to be realized, full \gls{interoperability} and combined analysis at the scale of millions to billions of stars will be required across all relevant surveys, which poses significant challenges in data management and \gls{software} systems, as described by \citet{Olsen_wp_372}.

\subsection{Compact Objects; Time-Domain and Multi-Messenger Astrophysics}

\citet{Graham_wp_377} highlight the explosive-transient discovery-space potential for \gls{LSST} combined with \gls{ELT} follow-up, which will only be realized if detection, filtering, and follow-up can be triggered rapidly by scientifically tuned \gls{software} systems. \citet{Kirkpatrick_wp_123} argue for increasing the transient and variable science return of the NEOCam mission through investment in the \gls{software} infrastructure needed to detect, monitor, and alert on non-moving (i.e. non-Solar system) variable sources. This is an example of how \gls{software} alone can qualitatively change the scientific opportunity space of a given survey/mission.

\citet{Cowperthwaite_wp_402} argue for the importance of ``target-of-opportunity'' observing with \gls{LSST} to follow up on \gls{LIGO} gravitational wave triggers in search of a counterpart. This points to the need for sophisticated real-time data-management \gls{software} systems such as \gls{LSST}'s to be implemented in ways that are flexible to the development of new and potentially unanticipated operational modes.

Binary systems with compact-object components provide ``astrophysical laboratories'' that will be central to many time-domain and multi-messenger applications in the coming decade. \citet{Maccarone_wp_251} describe the scientific potential for increasing the sample of known stellar binaries with a black hole component, and highlight the importance of time-domain photometric surveys such as \gls{LSST}, \gls{ZTF}, \gls{ATLAS}, PanSTARRS for identifying candidate systems through analysis of light curves to identify ellipsoidally modulated binaries and optically-outbursting X-ray binaries. \citet{Eracleous_wp_16} describe the role of \gls{LSST} and \gls{ZTF} in catching the disruption of white dwarf stars by a black hole companion, which can be further informed by \gls{LISA} observations when available. \citet{Littenberg_wp_44} and \citet{Kupfer_wp_210} describe the importance of \gls{LSST}, \gls{ZTF}, Gaia, BlackGEM, SDSS-V, and \gls{DESI} for identifying ultracompact binaries that will be potential future persistent gravitational wave sources for \gls{LISA}. In all these cases, algorithmic time-domain analysis and discovery implemented through science-driven \gls{software} systems will be essential.

\citet{Palmese_wp_346} highlight the potential for large spectroscopic surveys to provide redshifts for hosts of future gravitational-wave inspiral sources, both ``bright'' and ``dark''. These redshifts will enable ``standard siren'' cosmology in combination with the inferred intrinsic parameters of the \gls{GW} sources. This points to the need for spectroscopic surveys to make their data archives fully accessible.

Cutting across several of the scientific topics above, \citet{Chang_wp_482} provide an overview of ``cyberinfrastructure'' needs for multi-messenger astrophysics in the coming decade.

\subsection{Galaxy Evolution}

Large extragalactic surveys and their associated data archives are a key resource for advancing our understanding of galaxy evolution. \citet{Behroozi_wp_141} highlight the importance of large surveys, accessible data archives, and open \gls{software} for advancing our knowledge of galaxy evolution through the particular method of empirical modeling. \citet{Dickinson_wp_595} envision a future spectroscopic galaxy survey that would provide a highly complete SDSS-like sample across multiple redshifts, which would enable a comprehensive study of the coevolution of galaxies and their stellar populations with the formation of dark matter halos across cosmic time. Additional galaxy-evolution (and cosmology) science drivers are discussed below in Section~\secref{sec:multiprobe} in the context of combining data from multiple surveys and facilities.

Multiple quasar science opportunities in the next decade will be driven by survey-scale and data-intensive methodologies. \citet{Shen_wp_302} describe the role of large, time-resolved spectroscopic surveys to map the structure and growth of quasars through the method of reverberation mapping. \citet{Fan_wp_137} highlight the prospects for data mining in \gls{LSST} and \gls{WFIRST} for large samples of high-redshift luminous quasars, which can probe the coevolution of galaxies and their central SMBHs at early times. \citet{Pooley_wp_455} highlights the role of \gls{LSST} as a resource for discovery of strongly lensed quasars which can uniquely probe the dark-matter fraction in the lensing galaxy, while \citet{Moustakas_wp_539} describe the role that these same systems can play in reconstructing the detailed structure of quasars themselves.

\citet{Lehner_wp_524} highlight the importance of high-quality spectroscopic reduction pipelines and accessible data archives to maximize the science potential of high-resolution spectroscopy on large ground-based telescopes to trace the evolution of the intergalactic and circumgalactic medium over cosmic time.

\subsection{Cosmology and Fundamental Physics}

With its goal of understanding the contents and evolution of the universe as a whole, cosmology has driven many of the recent advances in ``big data'' astronomy. This trend is likely to continue through the 2020s. Many Astro2020 science white papers describe planned and proposed missions for which robust data-processing and data-management systems will be essential baseline requirements. These projects require not just basic management of petascale data, but also the automated execution of sophisticated inference algorithms---for galaxy shapes, photometric and spectroscopic redshifts, selection functions---across their entire datasets.

\citet{Slosar_wp_111} provide a broad overview of prospects for ongoing study of dark energy and cosmology with large-scale surveys. \citet{Dore_wp_379} give an overview of the cosmological science capabilities of \gls{WFIRST} via the channels of weak lensing, galaxy clustering, supernovae, and redshift-space distortions. \citet{Wang_wp_563} describe the dark-energy science potential of multi-tracer wide-field spectroscopic surveys that achieve higher completeness and spatial density than existing or planned surveys. \citet{Slosar_wp_112}, \citet{Ferraro_wp_85}, and \citet{Meeburg_wp_122} describe the prospects for constraining models of inflation and early-Universe physics through the signatures of primordial non-Gaussianity in large-scale structure surveys. \citet{Pisani_wp_51} describe the potential to constrain dark energy, neutrinos, and modified gravity in cosmic voids within densely sampled redshift surveys. \citet{Dvorkin_wp_75} describe the prospect for measuring the absolute neutrino mass scale through several large-scale observational channels. \citet{Rhodes_wp_129} envision the definitive large-scale structure survey to map the three-dimensional position of all galaxies and dark-matter halos in the visible universe. \citet{Geach_wp_608} envision a future wide-field spectroscopic survey in the sub-millimeter which would cover redshifts 1--10.

Large surveys and their associated \gls{software} and data systems will likewise be central to the quest to understand dark matter in the coming decade. \citet{Gluscevic_wp_150} describe the potential for galaxy and Lyman-alpha forest surveys, in combination with modeling and simulation of baryonic effects, to constrain the nature of particle dark matter. \citet{Bechtol_wp_230} describe the dark-matter science potential of \gls{LSST} on its own and in combination with spectroscopic facilities. Other channels for constraining particle dark matter with large spectroscopic surveys of galaxies and Milky Way stars are described by \citet{Li_wp_279}. \citet{grin_wp_XXX} describe how a combination of \gls{CMB}, optical, infrared, and gravitational wave observations will contribute to our understanding of ultra-light dark matter candidates.

Survey-scale cosmological science in the 2020s will also leverage machine learning (\gls{ML}) supported by large and well-calibrated datasets. \citet{Ntampaka_wp_21} describe recent applications of \gls{ML} to a diverse range of applications in cosmology, and highlights some of the most significant opportunities for \gls{ML} to increase the scientific return from \gls{LSST}, \gls{SKA}, and other major future projects.

\subsection{Combining Multiple Probes of Cosmology and Galaxy Evolution}
\label{sec:multiprobe}

A central theme of many Astro2020 science white papers at the interface of galaxy evolution and cosmology---and one that will significantly drive requirements for the computing, data, and \gls{software} systems of the 2020s---is the need to combine and co-analyze data from multiple major surveys. These use cases imply requirements for data accessibility, \gls{interoperability}, and mobility between data-hosting locations. They will also drive the astronomy and cosmology communities to leverage the capabilities of research-supercomputing and commercial-cloud computing providers in new ways.

\citet{Newman_wp_399} and \citet{Mandelbaum_wp_404} describe the synergistic potential for deep and wide-field survey spectroscopy to enhance the dark-energy science return from \gls{LSST}. \citet{Chary_wp_55}, \citet{Eifler_wp_463}, and \citet{Rhodes_wp_224} describe joint analysis approaches for \gls{LSST}, Euclid, and \gls{WFIRST} that would enhance the resulting weak-lensing and galaxy-clustering cosmology measurements of these missions. \citet{Capak_wp_521} describe the scientific benefit from coordination of ``deep field'' regions across multiple surveys and multiple wavelengths. (Here, standardized data and metadata formats will be necessary not only to realize the scientific potential of diverse datasets in common areas of sky, but also to enable discovery of existing datasets and coordination of planned future deep-field campaigns.) \citet{Furlanetto_wp_161}, \citet{Cooray_wp_59}, and \citet{Cuby_wp_401} describe the potential for combining galaxy surveys (space and ground-based), 21cm surveys, and other probes to obtain a more detailed picture of the epoch of reionization. \citet{Mantz_wp_308} describe the importance of combining multiple large surveys across wavelength for the selection of uniform and significant samples of high-redshift galaxy clusters.



==> old_text/software.tex <==
\section{Software \Contact{Arfon Smith, Erik Tollerud}}\label{sec:software}

\Contributors{Arfon Smith <\mail{arfon@stsci.edu}>, Erik Tollerud <\mail{etollerud@stsci.edu}>, Kelle Cruz, Stuart Mumford, Nirav Merchant, Gautham Narayan, Alex Drlica-Wagner}
\bigskip

\input{caveat}

In the Petabyte era, all projects are software projects --- that is, sophisticated software is necessary throughout the system for essentially any scientific output at this scale. That said, the term \gls{software} can mean many things to many people. Other Sections (e.g. \secref{sec:science}, \secref{sec:data}, \secref{sec:algorithms}) discuss the \emph{content} of this software, and the software ``infrastructure'' components and how they fit together are discussed in more detail in \secref{sec:tech}. Here, by contrast, our focus is on the process by which software distributed to and used by the astronomy community is built and funded. We particularly focus on \gls{community software} as it is the most relevant for the community to be involved in and for funding agencies to support. Note that that while clearly critical to the process of software development, relevant career and workforce issues are discussed separately in  \secref{sec:iwft:software}.

% Software can be written by anyone, but in order for it to qualify under our definition for this chapter, it must be distributed to, and used by the astronomical community.

\subsection{Recommendations}

% continuous improvement instead of maint

% project-level upstreaming needs a breakout: funding makes recruiting easier. Could also be co-shared pots of money to enable better generalization?

% * maybe have separate funding streams for generalizing
% * maybe say "need to upstream" rather than "bonus for upstreaming"
% * should the recc be "increased awareness" of the importance of upstreaming?
% * adding money doesn't help b/c it'll just be moved for something else

% * idea: move the "project "

% * Section title idea: ``Broader software impacts''? <- meaning the broader *science* community, "software ecosystem"
% * Don't let projects de-scope software?  HOLD ACCOUNTABLE.  Including upstreaming. But also educating managers?

% * Code should be developed and planned as part of an open ecosystem across the astronomy community

% * Review of data management systems should include specifically how well they fit in the wider ecosystem

%\WOM{We need to shift the culture toward open software - this is the current way of the world so we are enforcing this in astronomy. We need to educate ourselves all the way up the management chain on the beneficial broader software impacts of open collaborative development. We also need to ring fence software budgets in the overall project proposals. Should we also consider in annual personnel reviews and interviews people open source contributions?}

% Careers/prestige: who are these aimed at? Journals, departments, data centers?  Data centers may be better about that, so that makes it even more important

% EPD: who is this aimed at? Might want to move completely to workforce

\nrec{Software}{Agency}{Long}{swmoney1}{Funding for \gls{software} development in existing grant programs}{Software that enables science should be allowable as a sole deliverable for all existing funding programs (e.g. \gls{NSF} \gls{AAG}, \gls{NASA ROSES}, postdoctoral prize fellowships). It should not be necessarily coupled to a specific science effort, as long as the \gls{software} is of demonstrable use to the scientific community.}

\nrec{Software}{Agency, Astronomer, Technologist}{Medium}{swmoney2}{Funding for sustaining core astronomical ``community infrastructure'' projects}{Funding agencies and the community as a whole should support funding of domain-specific community-developed \gls{software} projects e.g. Astropy project, SunPy.  Such projects should be recognized as vital infrastructure and placed on an equal footing to physical facilities such as national observatories.  This support should be available for domain-specific \gls{software}, rather than funding being primarily tied to interdisciplinary applicability. It should also be allowed to fund community-development efforts in addition to actual code development.}

\nrec{Software}{Agency, Manager, Astronomer}{Short}{swecoplan}{Cultivating a sustainable research \gls{software} ecosystem}{Funding agencies should include as part of their review criteria for all astronomy grant programs: 1) A plan for how \gls{software} (not just data) will be managed to support the science of the grant, 2) How proposed \gls{software} development fits into and supports the wider ecosystem of available tools, and 3) Favor programs that propose developing \gls{community software} as part of their funded activities. These same goals and considerations should also be considered and acted on by the broader astronomy science community when e.g. working as grant review panelists.}

Note that cultivating a research \gls{software} \emph{workforce} is critical to all of the above. Hence, while not detailed in this Section, the recommendations of \secref{sec:iwft} are also as critical to the discussion in this section as the above.

% Note, this is likely moving to the workforce section.
% \rec{swcareers}{Career recognition}{Software should be recognized as a core product of modern astronomical research. Software outputs should be considered in all aspects of academic performance appraisals, career applications, tenure review cases. This is discussed in detail in \ref{sec:iwft:careers}.}

% \rec{swprestige}{Software Prestige}{The astronomical community should find ways to increase the visibility and prestige of software. Potential mechanisms include offering community prizes, providing first class support for citation in publications, indexing software citations, and developing metrics for evaluating impact. This is discussed in detail in \ref{sec:iwft:cookies}.}

% \rec{swedu}{Education and professional development}{Access to education and training for students and professionals which enable scientific grade software which adhere to software development best practices.This is discussed in detail in \ref{sec:iwft:software}.}

\subsection{Why shared \gls{software} matters, today and in the next decade.}

In this chapter, we argue that the Petabyte era of discovery in astronomy means that the role of \gls{software} is increasingly important and that well-organized, well-maintained \gls{software} serves to shallow the learning curve, enable scientific investigation, and lends confidence to scientific results.
To set scope, though, we emphasize this mainly applies in the context of shared \gls{software}.
That is, the ``throw away'' analysis script written, say, by a graduate student when writing their thesis and never shared with anyone else does not count for this discussion.  However, that changes when the same student shares that script with their collaborators, makes it available online, or contributes it to The Astropy Project, rOpenSci, or another open \gls{community software} resource. Such an act makes the software part of a community process, and the astronomy community is the target of this discussion.  Hence, in this chapter we are focused on \emph{shared} software.

%What do we mean by software, especially for projects like LSST and WFIRST? We want to educate our audience on how broad the range of software for data intensive discovery is.

\subsubsection{Software is everywhere}

\begin{quote}
    ``\textbf{Software is a central part of modern scientific discovery}. Software turns a theoretical model into quantitative predictions; \gls{software} controls an experiment; and \gls{software} extracts from raw data evidence supporting or rejecting a theory'' - Gaël Varoquaux, scikit-learn\footnote{\url{https://scikit-learn.org}} creator, \citep{varoquaux, scikit-learn}.
\end{quote}

Software is an integral, and growing part of the scientific endeavor: It is responsible for driving the control systems of instruments, the operation of surveys, the processing of raw data products, the extraction of physical parameters, and the theoretical modeling of physical systems, \gls{software} is critical to all parts of modern computational research. Indeed, `Software is eating the world' \citep{andreesen}. This reality is well-recognized by the scientific community: In a survey carried out in 2009, more than 2000 scientists reported that \gls{software} was either important or very important to their research, and that it would be impractical for them to carry out their research without it \citep{Hannay2009}.

The rapid increase in the size and complexity of astronomical experiments and the data they produce has led to an increasing demand for astronomical software. An illustration of this point is the \gls{LSST} project and their allocation of 25\% of the construction budget (\$187M) for data management \gls{software}, infrastructure, and services\footnote{\url{https://www.nsf.gov/about/budget/fy2018/pdf/30b_fy2018.pdf}}.

Over the last decade, in a large part driven by broader changes in the cultural `norms' of modern \gls{software} development and a shift towards \gls{open source software} being `the new normal' \citep{opensourcedotcom, forbes}, the astronomical \gls{software} environment has changed rapidly: Large experimental projects (such as \gls{LSST}, \gls{JWST}, \gls{DESI}, \gls{DKIST}) are writing extensive code bases and releasing these tools as open source software\footnote{\url{http://github.com/lsst}}\footnote{\url{http://github.com/spacetelescope}}\footnote{\url{http://github.com/desihub}}\footnote{\url{https://github.com/DKISTDC}}. At the same time, individuals are becoming increasingly likely to distribute and share their code broadly with the astronomical community and mechanisms for publishing these \gls{software} products have expanded as a result \citep{aassoftware, githubzenodo, Smith2018, astroandcomp}. In this data intensive future, where \gls{software} permeates scientific investigation, it is critical that the contributions of \gls{software} developers are recognized and that individuals are provided with the necessary resources to succeed.

\subsubsection{Software encodes knowledge}

As datasets become larger and our analysis methods more sophisticated, an increasing fraction of the scholarly method is expressed in software. This presents opportunities and challenges. One potential opportunity is that the `centralization' of astronomy (i.e. the trend towards smaller numbers of large facilities, often with open datasets) means that any \gls{software} built (and shared) leveraging these facilities has a higher reuse potential. A major potential risk, identified by others \citep{Donoho2009, stodden2010}, is that as the fraction of our research method is captured in \gls{software}, if this \gls{software} isn't shared (e.g. as open source), reviewed, or tested, the \gls{reproducibility} of our science is increasingly at risk.


\subsubsection{Software for reproducibility}
% Gautham - feel free to edit - might benefit from some text on reproducibility being central to good science overall
As projects become increasingly complex, ever more discrete \gls{software} components are combined to produce analyses and data products. However, despite this complexity, much of the code being used is not documented, let alone complete with unit tests that can validate performance. These shortcomings can have real-world consequences, as illustrated by the failed Mars Climate Orbiter mission, where \gls{software} calculations were carried out assuming metric units, but navigation \gls{software} was programmed assuming imperial units, leading to a premature and fiery end to the mission in the Martian atmosphere. While this is an extreme case, it is an illustrative bounding case for more subtle problems in analyses that lead to biases which are not detected.  Such problems are surprisingly common even in the computational science literature \citep{Collberg16}, much less more applied fields like astronomy.  While progress has been made in developing technologies to improve this (e.g. easy and widely available \gls{software} repositories like GitHub, containerization technologies like \gls{Docker}, etc), many of these technologies are still aimed at early-adopters in science rather than the mainstream.
%We recommend, that in addition to providing high-level science data products, large projects move to providing containerized versions of their software stacks. We expect that this will facilitate not only code reuse between large projects, but also help validate analyses, and make sure the results are reproducible.

\subsection{Progress in the last the decade}

Many of the issues highlighted in this chapter are not new. In particular, we highlight a white paper from the Astro2010 decadal review with a similar scope: \citet{weiner09}. That paper discussed areas of concern and specific recommendations, some of which have improved materially, while others have seen little progress. We discuss the recommendations of that paper here to provide a historical context and guidance for the future.

\begin{enumerate}
    \item \citet{weiner09}: \emph{``create a open central repository location at which authors can release \gls{software} and documentation''}.  Enormous progress in this area has been achieved in the last decade. \gls{open source software} repositories, chief among them GitHub\footnote{\url{https://github.com}}, have become a defacto standard for storing \gls{software} in astronomy. The wider adoption of Python has improved the  packaging and release process due to the Python Package Index\footnote{\url{https://pypi.python.org}} and the ecosystem of easy-to-host documentation tools that support Python, like Sphinx\footnote{\url{http://www.sphinx-doc.org}} and ReadTheDocs\footnote{\url{https://readthedocs.org/}}. While these are not a perfect solution for some languages and science domains, the presence of a much larger and better-funded user base (open source industry \gls{software}) has made them stable enough to be adopted for astronomy's use and can likely continue to do so for the foreseeable future.
    \item \citet{weiner09}: \emph{``Software release should be an integral and funded part of astronomical projects''}. Progress in this area has been mixed. While large efforts for this decade like \gls{LSST}, \gls{JWST}, \gls{DESI} or \gls{DKIST} have large first-class \gls{software} components, many smaller projects or individual grant-level efforts continue to treat maintainable or reproducible \gls{software} as an afterthought to be dealt with in whatever time is left over by graduate students or postdocs rather than a necessary part of the scientific endeavour. While funding agencies like the \gls{NSF}, \gls{DOE} and \gls{NASA} have required data management plans, there has been less progress on establishing firm requirements or expectations of sustainable \gls{software} (although a recent NASA-driven consideration of these issues is available in \citealt{nasaosp}).
     \item \citet{weiner09}: \emph{``Software release should become an integral part of the publication process.'' and ``The barriers to publication of methods and descriptive papers should be lower.''}. Considerable progress has been made in this area.  The \gls{AAS} journals now allow software-only publications on equal footing with more traditional science publications \citep{aassoftware}, and other major astronomy journals like A\&A and \gls{PASP} do as well.  New approaches to publication like the Journal of open source Software\footnote{\url{http://joss.theoj.org}} \citep{Smith2018} or the Astrophysics Source Code Library\footnote{\url{http://ascl.net}} are now providing alternate ways to publish \gls{software} that are indexed in \gls{ADS}.  Software archives like Zenodo\footnote{\url{https://zenodo.org}} now connect with GitHub to make publication of \gls{software} via \gls{DOI} almost frictionless \citep{githubzenodo}.  While there are still challenges in identifying how \gls{software} citation should work in these areas, tangible progress and recommendation is being made \citep{Smith2016}.  The ``cultural'' elements of ensuring these publications are viewed with the same level of value as other publications may also be improving, although concrete data in this area is lacking. While somewhat less progress has been made in ensuring open \gls{software} is a truly integral part of publication, the same resources noted above have made it much easier to preserve \gls{software} long-term.  More challenging is preserving the \emph{environment} \gls{software} has been run in.  While technologies like \gls{Docker} or virtualization provide a possible path, they have not been adopted widely across the community thus far, and represent a possible major area of development for the 2020s.
    \item \citet{weiner09}: {\emph{``Astronomical programming, statistics and data analysis should be an integral part of the curriculum''} and \emph{``encourage interdisciplinary cooperation''}}.  While some progress has been made in this area, there are many challenges remaining.  We defer further discussion of this to Sections \secref{sec:iwft}, \secref{sec:epo}, and \secref{sec:algorithms}.

    \item \citet{weiner09}: \emph{``more opportunities to fund grass-roots \gls{software} projects of use to the wider community''}. While such projects have grown remarkably in the last decade (see \secref{ssec:opendev}, major challenges still remain in \emph{funding} such projects in a sustainable manner, and these form the core of some of our recommendations.
    \item \citet{weiner09}: \emph{``institutional support for science programs that attract and support talented scientists who generate \gls{software} for public release.''}. Some of the elements of this recommendation have grown with the advent of ``Big Data'' and ``Data Science'' academic positions in astronomy.  There has also been a growing recognition of the importance of research-oriented \gls{software} positions, particularly in Europe \citep[e.g.][]{rse}.  However, there are very few viable pathways for researchers who develop \gls{software} of broad use as part of their research program if it is not considered a ``hot'' field.  Because, as this book demonstrates, there are likely to be \emph{more} areas where deep \gls{software} expertise is critical to science in the coming decade, the need for the field to nurture such career paths will only become more acute.  Hence this is also a key element of our recommendations.
\end{enumerate}

There is one final distinction to be highlighted relative to the last decade: it is clear that \gls{software} has become more mission-critical than in the past. As the other chapters of this book highlight, in the coming decade(s) large-scale science will require larger and more complex software.  These generic concerns about \gls{software} development are therefore multiplied across the deeper layers of \gls{software}, making all the issues more broadly applicable. The urgency in addressing these issues will only grow in the coming decade.

\subsection{Community \gls{software} as a force multiplier}
\label{ssec:forcem}
% , especially for large, community datasets
% Gautham - feel free to edit - I've added a note about not necessarily open source, but this does read like open source manifesto in part
Collaboratively-developed \gls{community software} has an increasing large impact throughout the astronomy community.  For example, the whole scientific \gls{software} ecosystem in Python \citep[the most popular language in astronomy][]{momcheva15} is built on community-developed \gls{software} like NumPy \citep{numpy}, SciPy \citep{scipy}, Matplotlib \citep{Hunter:2007}, or other parts of the so-called ``NumFOCUS Stack''. More domain-specific projects such as Astropy project\citep{astropy1, astropy2} and SunPy \citep{sunpy} capture the expertise of a broad range of astronomers, and have a wealth of features that cannot be reproduced by solitary researchers.  While the mere existence of such \gls{software} open to all to use are immediately apparent, there are several ancillary benefits to such \gls{community software} efforts:
\begin{itemize}
    \item The more the community participates, the more the project will reflect their specific needs and applications, even if it is built on a more general framework.
    \item The code is typically inspected by more people, and many eyes make all bugs shallow \citep[i.e. code problems and their solutions will be quickly found][]{raymond01}.
    \item There is usually more documentation available because of the free energy to specialize on such tools, and a larger base to help support new users.
    \item It is easier to train scientists to help produce professional-quality \gls{software} if they are supported by a core of professional engineers. Community projects provide a larger-scale social understanding of how that interaction can happen.
    \item These projects speed up the cycle of science by providing useful implementations for common tasks, freeing up researchers to work on their specific science.
    \item When built as part of an underlying broader ecosystem, \gls{community software} often gains the direct benefit of contributions ``upstream'' e.g. improvements in core math libraries made by computer scientists can flow down to astronomy without any direct effort in astronomy.
\end{itemize}

Together, these factors mean that the impact of code developed by a community is multiplied by further contributions from other sources to the same ecosystem.

We note that the community developed \gls{software} need not strictly be open source, though the majority of these projects are. The benefits of community development extend to both open and closed source projects, the primary difference being that the potential size of an open project is by definition larger than a closed one, and most of the above scale with community size.

\subsubsection{Open development/Open collaboration}
\label{ssec:opendev}

While a substantial fraction of software in Astronomy is now \gls{open source software}, and has been for decades, a major development in recent years has been the growth of \gls{open development}. This form of collaboration software development accepts and in many cases depends wholly on contributions from the wider community to the software project. Development of the code and discussion around that code is conducted in the open using industry-standard platforms like GitHub or GitLab, and in most cases policy discussions and decisions also occur in the open, or example on a public internet mailing list.  The chief examples of projects like this in astronomy are The Astropy project and SunPy.

This kind of development model is not limited to astronomy projects, there are many examples of large scale \gls{software} projects which are entirely developed in the open, the largest example of which is the Linux kernel. Developing \gls{software} in this way introduces technical and sociological challenges, which have been met by \gls{DVCS} tools such as \gls{git}, online collaboration tools such as GitHub that enable workflows which scale to many hundreds or thousands of contributors, and the hard work of organizers and code reviewers to set up and maintain a positive culture that enables contributions to continue.

These kind of open collaborations enable many different stakeholders (both astronomer-users and dedicated developers) to collaborate on a \gls{software} project, often from a diverse set of perspectives. While this is possible with non-open developed \gls{community software}, it is often much harder because it requires an added layer of communication between ``users'' and ``developers'', while in \gls{open development} these are the same community. This makes the \gls{software} more valuable to both the contributors and the community more than the sum of the individual contributions, as it reflects the needs of the many rather than the one. It also means more work can be done with less funding, because the efforts of individual contributors are pooled into a ``neutral'' space that can arbitrate via the community process. Moreover, the open nature of the collaboration means that stakeholders have the ability to drive the direction and priorities of the project simply by contributing to it. Because many of these stakeholders are the users themselves, it also can serve to optimize the applicability-to-effort ratio.

\subsection{Community \gls{software} problems and solutions}

With the above in mind, there is incongruity between the increasing importance of \gls{community software}, and the funding available for such projects. In particular, the future of many widely used projects that are effective force-multipliers, including \texttt{astropy}  and services such as \url{astrometry.net}, are uncertain. These major community projects are generally unfunded despite the vital role they play for astrophysics as a whole. While many feature ``in-kind'' contributions from user missions (as discussed above), such support depends on the vagaries of mission priorities rather than the needs of the community itself (as discussed below).

Hence, the benefits outlined above cannot be realized if such efforts are not supported by funding agencies, large missions, and indeed the astronomical community as a whole. Currently incentives are not in place to encourage community efforts: indeed in some cases such \gls{software} development is either not allowed by a grant program, or tacked on as an afterthought. (``Oh, we'll probably have my grad student build that reduction pipeline on the way to their thesis.'') Where \gls{software} grant programs do exist, they often focus on building specific applications into interdisciplinary tools (e.g. \gls{NSF} \gls{CSSI} and \gls{DIBBs}), rather than applying general \gls{software} to specific domains. They also as a rule do not emphasize \emph{community-building} elements like contribution policy documents, documentation of user workflows, or community coordination. Hence, while specific recommendations of what platforms for development are useful are not likely to be relevant in 10 years (and indeed are often counter-productive - see \secref{sec:swalive}), our recommendations focus on incentives for pro-social behavior by missions and individuals. This will be critical to keeping up with the ever more software-rich Petabyte era, and this is precisely what the recommendations of this chapter aim to do.

\subsection{Software is alive}\label{sec:swalive} % refered to in technology

\label{ssec:sw_alive}

\begin{quote}
    ``This open source stuff is free. But it's free like a puppy. It takes years of care and feeding.'' - Scott Hanselman on the death of nDoc \citep{ndoc}
\end{quote}

The grant-funding model for academia fosters a picture of all work as limited to a fixed time horizon, shared astronomical \gls{software} often lives as long as it is useful.  This can be far longer than any individual researcher or developer, and as a result the \gls{software} takes on a life of its own.  Like any living thing, however, this \gls{software} will not survive without proper care and feeding, and without evolving to adapt to continually changing environment.



\subsubsection{The \gls{software} stack is always changing. We need to be adaptable.} \label{sec:stack}

Sustainability is a necessary but not sufficient condition for \gls{software} to survive. Even with maintenance, the entire \gls{software} ecosystem is constantly evolving. A clear example is Python replacing \gls{IDL} as the most popular programming language within astronomy \citep{momcheva15}, despite many of the elements of the \gls{IDL} Astronomy Library being maintained. Similarly, many of the features of \gls{IRAF} are now being provided by widely used community projects such as Astropy project, despite the long history of \gls{IRAF}. New \gls{software} like this generally evolves because they can tackle problems that were not addressed previously, either by making the coding easier or taking advantage of other developments in the wider technical world (discussed more above). For example, resasons for the change from \gls{IDL} and \gls{IRAF} to Python are the lack of license fees, the extensive open source ecosystem of libraries for scientific computing, and the easier learning curve of the latter (due to more broad usage).

However,  the disruption caused by the evolving \gls{software}  ecosystem can be disruptive because it comes at the cost of requiring significant retraining and refactoring. In this way, the need to be adaptable to changing developments in \gls{software} can appear to be in tension with the need for well-validated \gls{software} for research. There is indeed always a cost-benefit analysis for changing technologies that most include this concern as much as the benefits that may result.  But consideration must be made that this disruption can be ameliorated by continuing education programs for researchers at all levels.  Examples include \gls{AAS} workshops, introducing astronomers to the up and coming \gls{software} projects and to highlight long-term trends, such as which projects are growing in support vs which are now largely unmaintained.  There are further more focused recommendations in \secref{sec:iwft} for keeping the community on top of such changes. Hence, the disruption caused by the continuous evolution of the \gls{software} stack should not be feared, but rather welcome for its potential to improve our own research.


\subsubsection{Software needs to be sustainable}

\label{ssec:soft_sustain}

Any \gls{software} that is meant to be used more than once requires maintenance. Data sets change (or grow to Petabyte scale), bugs are discovered, computer architectures change, and users change their understanding of the intent of the software. This leads to the concept of \gls{software} sustainability: practices both within the \gls{software} itself and of those who develop it that make it practical to maintain the \gls{software} for an arbitrarily long time.  For astronomy \gls{software} to be sustainable~\citep{wssspe51, wilson14}, it should:

\begin{enumerate}
    \item Be both  testable and tested (i.e. it is correct and that correctness can be checked by anyone).
    \item Be readable and useable by multiple people (i.e.  it can  evolve to fulfill its intent over time as development and scientific conditions change).
    \item Have a viable pathway to be maintained past the original author (i.e. survives uncertainty).
    \item Be able to respond to users' needs, even if they change over time (i.e. supports relevant concerns).
\end{enumerate}

As outlined in \secref{sec:stack}, even for \gls{software} that is maintained, for example by a third party organization (e.g. Harris Geospatial Solutions for \gls{IDL}) does not guarantee future usage of this technology within astronomy \citep{momcheva15}. As astronomy shifts towards a more community-developed, open source set of tools, it iss critical that different constituents of the astronomy community develop an understanding of the origin of this \gls{software} and how they might be able to participate in its development, maintenance, and long term sustainability:

\textbf{Software consumers (individual astronomers)}: Most individual researchers are \emph{consumers} of \gls{community software}, that is, they make heavy use of the \gls{software} tools developed by their peers but do not routinely participate in the development of the software. Like most community-developed open source projects, this is the norm and is acceptable. However, complete ignorance of the origin of the \gls{software} they are using creates a risk to the sustainability of the projects and individuals responsible for creating the software. For example, if they do not realize the \gls{software} they are using comes from other researchers, they may not support hiring, tenure, etc of those who build that \gls{software}, thereby stopping them from producing and maintaining the \gls{software} itself.  We believe therefore that even as \gls{software} consumers, astronomers should increase their awareness of the origin of the \gls{software} they are using and realize that they have an important role to play in the community by 1) providing feedback to \gls{software} projects by filing bug reports, feature requests, feedback on existing tools, and perhaps contribute other resources like documentation if they have relevant expertise; 2) recognizing that \gls{software} is created by \emph{people}, and that supporting the work of their peers  (be it financially, socially, or even emotionally) who spend time creating these tools is necessary for the tools they use to even exist; and 3) recognizing and advocating for the broader concept that using a shared set of community tools can improve all of science for less money.
\newline

\textbf{Individual \gls{software} creators (individual astronomers and engineers)}: While these are the bread-and-butter \emph{of} these community efforts, they are not without shared responsibility here.  Specifically, the builders of community have a responsibility for being aware of the community they are building for.  E.g. they need to remember that the user community typically does not have as much technical expertise and therefore requires their \emph{help} to both learn how to use the \gls{software} and understand why it is useful. They also need to understand the unique responsibility that creating \gls{software} sustainably is work (see the above subsections) and must either agree to such work or communicate clearly to their potential users that they cannot do it without help.


\textbf{Institutional \gls{software} creators (projects/missions/facilities)}: Observatories and missions (e.g. \gls{LSST}, \gls{JWST}, \gls{DKIST}), especially in development \& construction phases, spend significant resources developing \gls{software} both for internal operations but also for their community to analyze and interpret data products from their facilities. These \gls{software} creators need to be incentivized to \emph{upstream} (i.e. contribute back new innovations to \gls{community software} packages) their \gls{software} where possible, thereby contributing to the large ecosystem of \gls{software} available to the general astronomy community. As discussed earlier in \secref{ssec:forcem}, \gls{community software} can be a force-multiplier when done right, but in order for this to happen, \gls{software} projects must recognize their role in the \gls{community software} ecosystem and shift towards being active contributors rather than consumers/users of community software.


% \subsection{Random notes}

% Need to say that software is not just "what my grad student writes" but also LSST DM, etc. Also need to make clear that software *is* infrastructure, rather than the two being separable.

% We need to move towards more open source but not mandate. Transparency, sustainability, etc...


% Things we need to reference: the NASA open code policy, Ben W's 2010 WP, ...

% These materials have broad utility, and are not limited to astrophysics.


% Tentatively: recommendations below contain ideas we should articulate but maybe not concrete recommendations?

% Something about Astrophysics Source Code Library

% \begin{itemize}

% \item open source should be the default. Projects should have to justify any deviation from open source.
% \item Grants/funding sources should be available to help community management including contributor onboarding, project management etc.

% \item Open access for software and data with the publications
% \item Lower the standard and methods for software sharing
% \end{itemize}





% \AMS{Here are some ideas for topics we might want to cover. These are just suggestions at this point so feel free to suggest alternatives etc.}

% \AMS{As a reminder, I think in all cases if possible, we should be framing software and services in terms of turning `Petabytes into science'}

% \begin{itemize}
% \item Software encoding knowledge: We probably want to say something about the fact that software, especially for data intensive astronomy, encodes deep expertise and can be a major academic contribution. In fact, as research fields become more computational, and an increasing fraction of the scholarly work (algorithms/methods, statistics etc.) are encoded in research software, without software publishing, we run the risk of research results are becoming increasingly irreproducible (\citep{Donoho2009}\url{http://gael-varoquaux.info/science/publishing-scientific-software-matters.html}).
% \item Software development, open source, `open collaborations': AMS - IMO the future of software development in astronomy and astrophysics is and open source one, at least for major pieces of software such as tools developed by facilities/projects/large collaborations. We could discuss here a few case studies both within astronomy (e.g. Astropy) and outside. I'm pretty sure Erik T. Will want us to discuss open collaborations too, that is, projects that are receptive/welcoming to new contributors.
% \item Sustaining open source/community software: If we end up writing about open source, we should spend some time talking about where it's most effective, some of the challenges maintaining it (i.e. access to funding), sustaining the careers of those individuals writing software (might just want to cite the workforce section here). \WOM{I think LSST has struggled in this area - it is open source and  welcoming but as you point out in the first bullet this stuff is hard and the price of entry is high plus we must value efficiency sometimes over elegance. Now perhaps we will have many more contributors when there is LSST data but it would be interesting to address this aspect as well.}
% \item Software interoperability: We might want to talk about the challenges of combining software from different systems (e.g. LSST and WFIRST) for e.g. joint pixel processing. Each project develops in a silo not necessarily paying attention to the other project which means that combining the tools is (probably) harder than it should be.
% \item Perhaps we should also sketch out the landscape of software for data intensive astronomy. For example, user facing tools, back-end services, services (e.g. brokers), software-defined infrastructure, software that controls infrastructure...
% \item Service oriented astronomy: \AMS{years ago I wrote about the idea of `Service oriented astronomy' (\url{http://arfon.org/on-the-possibility-of-service-oriented-astronomy/index.html}) which might be interesting here}. Essentially, an ecosystem of tools/services deployed around common infrastructure/datasets. An example of this would be broker services deployed to enhance the LSST alert stream (or any transient/event based service)
% \end{itemize}

% \begin{enumerate}

% \item The software stack is always changing. Python is the big thing now, which has advantages, but might not always be.  We need to accept the reality that things change, but we won't dwell on the "multi-decade horizon" (i.e., impossible-to-predict-trends) and instead focus on "now problems".  Also won't bother defining exactly what software we mean - it's everywhere, so the below applies broadly.

% \item open source/Open Dev (OSS) - why it's good for science, some pitfalls.  Include why large OSS projects are \emph{not} the same as IRAF/MIDAS/etc, and instead, enabled by new software collaboration tech, are a different ballpark.

% \item Impediments to OSS in astronomy:
% \begin{itemize}
%     \item Astronomers are used to rolling their own, don't trust things they didn't write.  Need to train them you can have your cake and eat it too.
%     \item Astronomers and particularly projects often take it as "I'll just use it" instead of "I'll join the community and help support it".
%     \item Astronomers/astro engineers are not used to having or being "users in a community".  Requires awareness of non-traditional "soft skills" and community-building
% \end{itemize}

% \item Impediments to OSS sustainability
% \begin{itemize}
%     \item It's hard to get money for OSS projects because they don't "live" anywhere in the traditional funding models (esp. NSF broader impact changes)
%     \item Career tracks for software specialists (or even 50/50s) are limited and lower prestige (e.g. "software instrumentation" is generally not a thing except in explicitly computational fields)
%     \item Hard to track sustainability so hard to solve it.  OSS maturity model + GitHub \url{https://github.com/github/maturity-model}?


% \end{itemize}

% \item SW and consistent versioning tools or containerization can be a huge sea-change in reproducibility.  See "software encoding knowledge" by AMS above for more details on this one


% \end{enumerate}

% open source as a force-multiplier.
% open source, if abused, is free like a puppy (or rabbits), rather than free like beer.


==> old_text/technology.tex <==
\section{Technology \& Infrastructure \Contact{William O'Mullane, Niall Gaffney}}\label{sec:tech}

\Contributors{William O'Mullane <\mail{womullan@lsst.org}>, Niall Gaffney <\mail{ngaffney@tacc.utexas.edu}>, JJ Kavelaars, Frossie Economou, Surajit Chaudhuri}

\bigskip
\input{caveat}

We discussed many of the challenges and potential technological and infrastructure innovations which could be future
solutions to current problems.
In these discussions, we concluded that the goal was not to predict future
problems and unknown technological solutions, but to unite and align
cross mission and research community \gls{cyberinfrastructure} needs.
We should standardize and  establish best practices based on those already found within missions.
These goals are best served
with a design that enables common user identity models, along with common data, \gls{software}, and infrastructure as services joining systems in a loosely coupled \gls{cyberinfrastructure}. This will drive the the field towards
a more interoperable cross mission \gls{cyberinfrastructure} by design rather than common \gls{API} and
piecemeal translation layers which we currently have.
This will enable developers to reach velocity more rapidly as they move between projects and missions since
they will be  more familiar with the  common development practices and reference architecture.



%\subsection{Establishing a community Wide Standardized Architecture} \label{sec:refarc}
\subsection{Commodity services and \gls{software} based community architecture} \label{sec:refarc}

%(JEK) I suggest changing the title of this subsection to "Encourage the use of commodity services and software that are widely used by science and industry"
%\WOM{A bit long how about "Commodity services and software based community architecture"}

% (WOM) Accepted !! Not clear what it replaces or do you mean for the intro above to the chapter ?.. (JEK) Alternative opening paragraph:
The astronomy and astrophysics community community have historically relied on the development and use of bespoke \gls{software} and hardware infrastructure to solve challenges related to the managing and analyzing datasets at a scale that was difficult to find in industry or other scientific domains.
These requirements are no longer unique and we have access to a wealth of open source \gls{software}, commodity hardware, and managed \gls{cloud} services (offered by commercial providers and federally-funded institutions) that are well positioned to meet the needs of astronomers and astrophysicists \cite{2019AAS...23345706M, 2019AAS...23324505B}.
By providing documentation and reference implementations of the “astronomy stack” using these technologies and making it easier for researchers and missions to access \gls{cloud} computing services, we can reduce operations costs, accelerate time to science, and increase the scientific return on Federally-funded research in astronomy and astrophysics.

Such an architecture/system will provide access to new  technologies for improved data \gls{interoperability}. For example to enable a system to recognize transients in multi-observatory data with more than just the photometry.  By housing such data as observing conditions, instrument bias, and even observation proposals within the system, developers can implement common layers at higher levels to provide common access  missions. This can be done without having to specify the complete system for gathering, managing, and formatting the data. Missions can enforce access to either sensitive or proprietary information through role based access control to the data. With a well designed service oriented \Gls{cyberinfrastructure}, cost can be minimized as less
%service-by-service
coordination will be needed to implement cross mission services.

%\such{The reference architecture has at least some elaboration for each layer, but none for "data level" - we need some explanation to add on what processing takes place at this level and what APIs are exposed}

%\such{One important component is data movement across cold to active storage, i.e., high latency to low-latency/interactive speed access.}

\begin{figure}
    \centering
    \includegraphics[width=1.\textwidth]{CI-Layers.png}
    \caption{An example a \gls{cyberinfrastructure} built on an Infrastructure as Code design model. Note that while this example does not have astronomy-specific tooling, our recommendations highlight the importance of developing astro-specific layers that are fully accessible to scientists in both  the application  and the graphical interface layers. \figref{fig:CI-LSST} presents an LSST/Astronomy instantiation of this.}
    \label{fig:CI}
\end{figure}\

\nrec{Technology}{Agency, Technologist}{Long}{cbra}{Develop a community wide architecture supporting Science as a Service}{
Agencies should fund the major missions to define and adopt a community wide supported data and compute service architecture with easy to adopt
components leveraging widely adopted infrastructure standards both in the community and in industry.
This "Infrastructure as Code" \citep{morris2016infrastructure} approach lowers the bar to entry
and allows for easier adoption of more standardized services that will enable large-scale
astronomical research in ways that are well demonstrated in plant genomics (CyVerse and Galaxy), natural hazards (Designsafe), and surface water research (Hydroshare).}

Many research communities have accelerated their time to discovery and lowered their cost of integration by adopting a
common community wide architecture that is supported
by multiple data and computational service providers. While
attempts prior to the past decade have been moderately
successful, the current shift in development across
industry to the support of smaller services rather than
monolithic data and compute systems allows for faster
and more cost effective deployment across communities.
By encouraging the definition  and production of  an astronomy focused, community wide reference architecture, perhaps by changing the funding structure, we can being to have a menu of services  easily implementable across service providers.  Design and
support for this infrastructure should be community driven, prioritized and funded, to allow for development of features across missions and science use cases.

%\such{As I read this section, it feels to be we are hinting at that the community should adopt the generic cloud infrastructure - IaaS, as well as managed services including PaaS and Serverless. In this connection, giving examples of your successful Commercial Cloud Usage Pilots will be helpful. I understand that you also want to cater to "in-house" Infra builders by urging them to converge to an architecture similar to Commercial Cloud providers and following standards that have emerged, but I wonder what would motivate them to change.}

%\such{A radical architectural approach, but in line with what is happening elsewhere, is organized in terms of services/micro-services that expose a REST API and we really don't worry if those services use on-premise infra or uses one or more of cloud providers. The power of such an architecture is for the community to share micro-services and build new services in a more agile way by relying on these micro-services. I wonder if there are opportunities in your world for "reusable" micro-services. During the meeting, it was mentioned that such an approach may be in line with what NIH is doing for funding}

Pictured in Figure \ref{fig:CI}  is the structure of a \gls{cyberinfrastructure} (\gls{CI}) that has been
used across multiple fields from plant and animal genomics
(CyVerse) to natural hazards engineering (DesignSafe). This shows the
layers of the \gls{CI} from the interfaces for service access exposed
at multiple levels, the common domain wide enabled services, and a collection of system level components that support the
higher levels of the \gls{CI}.
The lower down the diagram are commodity layers based on well established and supported
components. As one moves up from these layers, more abstraction can be done to
expose these pieces in domain or even question level interfaces. By making these
abstractions, more universal service can be developed that can be applied more globally
across the entirety of the \gls{cyberinfrastructure} as a whole.  An example of this would be
authentication, where each university or agency may provide their own authentication method
but unifying services like CILogin can bring those together to give global spaced
identity for a wide range of users based on disparate authentication systems.
By providing this structure along with a reference architecture of these System Services based on
well supported \gls{software} components, providers are easily able to both deploy and support these common services which enable
cross mission and center \gls{interoperability}. This structure also reflects how this architecture allows for greater reusability as one gets closer to the actual implementation of these
services while supporting greater flexibility and general usability as one works further from the core components.
This service architecture should be based on using standard reusable \gls{software} from many of the established standards developed outside of astronomy (e.g. common authentication mechanisms such as CILogin, standard data and metadata management systems).  Standard \gls{API} interfaces should also be used to expose these components to higher level \gls{API}s. Data
formatting and metadata structure can be exposed at the service level, allowing for
more data and metadata reuse.

\begin{figure}
    \centering
    \includegraphics[width=1.\textwidth]{CI-LSST.png}
    \caption{An example \gls{LSST}  \gls{cyberinfrastructure} built analogous to the \gls{CI} model shown in \figref{fig:CI}.}
% Original https://docs.google.com/presentation/d/16w5WVe-_xNLXWudNKqJu9IEKGDQ8oIB0eDiqWP_SUnE/edit?usp=sharing
    \label{fig:CI-LSST}
\end{figure}\

Such an architecture should be developed in a \gls{cloud} and
vendor agnostic manner.  When needed, vendor specific \gls{software}
or \gls{cloud} service can be integrated by a mission, but by isolating them in the \gls{cyberinfrastructure}  at the lowest level, their potential impact on the overall system is minimized. When possible, standard interfaces should be used to abstract out
these differences (e.g. standard object store access like \gls{S3}, standard database interfaces like \gls{ODBC}) and should be reflected in the reference architecture documentation. Where practical, computational environment abstraction layers such as
container technologies (e.g. \gls{Docker}) should be used to associate each
applications
computational requirements to the application rather than having to
enforce upgrades and updates across the complete infrastructure. Where
specific hardware environments are required (e.g. Google's Big Table
or Tensor Processors), it must be required that the interface to these
services leverage common \gls{API} or \gls{software} layers for access
(e.g. \gls{SQL} or Tensorflow) to allow for simpler migration to future or
separate vendor's systems.

%When it is not possible to be agnostic we must  define the migration path and cost for moving vendors later -  thus we  document the potential costs of lockin.

Many of the advances in the current data revolution have come about from the
broad adoption of commodity hardware and \gls{software} services being applied in
domain agnostic ways. While over a decade ago, astronomy was one of the first domains to
explore these technologies, the current momentum in the area is driven outside
of the astronomical field. Current technologies like Spark, Cassandra, Kubernetes, and
MongoDB were all created to support large data problems outside of astronomy but are
finding support in the astronomical community in a piecemeal manner. By shifting
the focus from local to a more distributed \gls{cyberinfrastructure}, such new technologies could be
implemented and leveraged much quicker than if each center had to support and
integrate their own solution, Further, by embracing and adopting a more commodity base infrastructure will allow current and future projects to choose and experiment with hardware alternatives such as \Gls{TPU}s, \Gls{FPGA}s, or Quantum computing as they become more commonplace or to integrate newer architectures that best suited to the problem.

There is a current tension or incompatibility with the direction of High Performance Computing \gls{HPC} to many more cores with not much more memory and large image processing which requires more throughput. Historically, systems designed for \gls{HPC} were
more suited to simulation as opposed to the embarrassingly parallel yet often memory intensive High Throughput Computing \gls{HTC}.
While \gls{HTC} does not get as much attention, it has been key to missions such as the Human Genome project,
\Gls{LIGO}, and \Gls{SDSS}.
While some are moving to bridge this gap (some in support of missions such as \gls{LIGO} and others because simulated data analysis is becoming
as complex as observational data analysis), agencies should continue encourage
and fund national computing centers to address the needs of both communities. Further, they should
enable simulated datasets to coexist within the infrastructure with observational datasets to support the full cycle of astronomical discovery. Finally, they should
formally adopt support for mission long computational support at these facilities
for all major missions.


We note the general idea here especially on the importance of \gls{cloud}  are compatible with  Rob Pike's thoughts\footnote{\url{https://drive.google.com/open?id=1kYsavh900I2o6z1lPfjFFXamyBkoEdCW}}.

Where ever possible, review of \gls{cyberinfrastructure} driven proposals should be ranked on both their immediate
impact to the field as well as their ability to sustain such impact through several technology and vendor cycles. Proposals should also be ranked based on their reuse and/or integration into the overall \gls{cyberinfrastructure} developed across the astronomical community.

%\ajc{Recommend open formats and software infrastructure where possible on the cloud. When it is not possible define the migration path and cost for moving. This is not to stop or recommend adopting a vendor but rather to document the costs of moving technologies}



\subsubsection{Identity and Access Management (\gls{IAM})}\label{sec:iam}
User identity is key to all data systems to date. In the
past, each mission has had its own \gls{IAM} system to provide data access
for embargoed or otherwise restricted data access and for accessing
services. With a more global \gls{CI}, this problem must be further abstracted to allow for the notion of identity of a user (aka authentication) and
permissions (aka authorization) for services and data. By separating
these pieces, identity can be brought from multiple sources (CI-Login,
OAuth, ORCID) while the permissions can be enforced by each provider.
All aspects of this \gls{CI} must embrace role based authorization for both data and services in a federated manor so that data and services
can be effectively orchestrated while not impacting site or mission
specific access restrictions. While the authentication may be global, each provider will enforce their own access roles for all users. As data analysis
moves into the petabyte and even exabyte scale across multiple missions
and multiple computational environments, it will be paramount to
for all members of the \gls{cyberinfrastructure} to share a common \gls{IAM}
infrastructure to allow for federated access controls for both
data and computational services.

Proposals and missions should be ranked on their adoption of
such an \gls{IAM} for data and for \gls{software} services. Further, by
creating a common \gls{CI} layer for identity, missions and smaller
services will be able to adopt and adapt the common system to
their needs, thus saving development costs for implementing and
finally supporting their own system.



% moved network to after data lakes...better order of things

\subsection{Data co-location and creating data lakes}\label{sec:coloc}

 \nrec{Technology}{Technologist}{Medium}{coloc}{Enable new scales of research through data co-location} {We must enable the co-location of data thus enabling large scale cross mission research. While some
 research are well supported using specific services, ones which require comingling data to produce new data products or results should be able to schedule access to co-located data in ways similar to acquiring new data.}

 Astronomy archives, especially in the USA, are somewhat fragmented. Though \gls{TB} scale permanently co-locating all data n one or more centers is technically possible it is probably not desirable nor socially possible.
In the \gls{PB} data era permanent co-location becomes less feasible, yet  researchers will require data lakes or reservoirs to house massive datasets and allow computations to be done across multiple missions and epochs
of data at scale. The data lake concept, where data from multiple missions and schemes
are temporarily co-located so as to allow codes to more tightly integrate with multiple data sources,
is the most attractive for researchers (who have become accustom to immediate data
access), the idea of a reservoir that can be filled and drained of data based on
the demand of users is one that will need to be explored due to the economical
viability of any one institution housing all the data.

Collocation is more than just \gls{interoperability} but  will also mean  generating
new formats  e.g. \gls{parquet} files (e.g.) to make dynamic
data frames and data services as demands change.  It will also mean generating
new data products across missions which are equally valuable for both
preservation and publication. Thus the lake is more than a simple pool of
storage, but should be operated similar to other key infrastructures in
the observational astronomical infrastructure.

Software and technologies change on timescales faster than a
decade (see also \secref{sec:swalive}) and  data centers need  to be agile enough to keep up.  One approach is to create
interoperability interfaces to allow data to be pulled
or pushed from managed repositories to dynamic data
lake environments where users can produce their own custom subsets mixing the available
datasets.
Data movement will not be simple (see also \secref{sec:net}) and to not be prohibitive
specific infrastructure would need to be supported and evolved.

While the immediately obvious argument for co-locating data is the potential for scientifically rich co-processing of heterogeneous data holdings (e.g. Euclid, \gls{WFIRST} and \gls{LSST}), the advantages do not end there. Co-locating large data holdings on a common commodity computing platform enables bring-your-code-to-the-data capabilities (sometimes referred to as Science Platforms or server-side analytics) to enable co-analysis of data from a single service without necessitating data transfer. For example, a single Jupyter notebook can present an runnable analysis drawing on separate datasets (e.g. a multi-wavelength analysis of a class of objects). Furthermore, co-locating data holdings allows the co-location \emph{and sharing} of services accessing those data holdings. That not only includes the possibility of collaboration in sharing a single \gls{API} service between data publishers, but also reducing the development burden of infrastructural services (for example, documentation infrastructure could be shared with multiple missions, migration paths to new operating systems are easier, etc). In an era where Infrastructure as Code engineering paradigms represent emerging best practice,
re-using the code that underwrites common astronomical services because they are developed within a common underlying infrastructure (such as \gls{Docker} containers orchestrated by Kubernetes) provides an avenue for fruitful ongoing collaboration between data publishers and better value for money for science infrastructure dollars.



\subsubsection{Network layer}\label{sec:net}
One area where Infrastructure as Code does not work is networking.  While data transfers
can be better optimized depending on the nature of the data being transferred, network
as a service will require optimizations often at the point to point level. Tools like
PerfSonar and others from Internet2 can help optimize connections. But these
have been used to optimize research done at the terabyte scale today. Where as in the
\gls{TB} scale it was possible sometimes to move the compute to the data (e.g. \gls{SDSS}), discovery often comes from the \gls{TB} scale data lakes. To meet the
demand for petabyte scale data motion as a service in a terabit network age, systems to support Just In Time data
delivery are needed for any large scale data collocation  and must be a part
of the support for the overall infrastructure of repository/cloud/data center
collaborations.  Computation on large datasets may need to be scheduled no
different than any other instrument used in observational astronomy.

We recommend funding projects in astronomy (and in other research domains) to
create the data management and migration layers and best practices that will
enable these new forms of observation. We also recommend that proposals show how they
will develop and sustain such services over the course of the mission and beyond.



\subsubsection{Vendor freedom}\label{sec:lockin}
When co-location of data holding and services on a \gls{cloud} platform is discussed, inevitable there are concerns raised about "vendor lock-in". These objections are often rooted in a misunderstanding of the nature of these services. First of all, these services often themselves share common open source technologies between them (for example there are a number of object store technologies that implement the an interface compatible with Amazon's \gls{S3} service). But more than that, the commercial landscape is designed around low barriers to change: Google Cloud Platform tries to acquire Amazon Web Services customers by making its services easy to switch to. Moreover all these platforms drive a service-oriented architecture that inherently results in more portable systems. In any case if one is concerned about vendor lock-in, in-house data center infrastructures are the worst possible choice: the inevitably lead to infrastructure-specific choices that are poor candidates for evolution, and they typically lack the effort to support ongoing refreshing of the technical stack thus creating on-going support burdens and a change-averse culture.
For example, \gls{LSST} is a project that will go into operations in 2022, and yet \gls{LSST} \gls{DM}  are frequently called on to support CentOS 6, an operating system released in 2011, because that is the only \gls{OS} some university in-house clusters support for researchers.


\subsection{Operations}\label{sec:ops}
\nrec{Technology}{Agency}{Short}{fundops}{ Enable support for full mission life cycle including long-term data products } {Agencies should revisit the model separating funding and
requirements for development and operations of large scale missions for which the data and services are key deliverables as well as steel and concrete.  Such services are under
continual development and integration and, in the current environment, can not simply be
maintained in the same way physical facilities are.}

A more operations oriented view of construction by funding organizations would lead to facilities which are more cost effective to run.
Recognizing that \gls{software}  and \gls{cyberinfrastructure} development work is distinct  from concrete and physical facilities  would also help to make more maintainable and agile \gls{cyberinfrastructure}.
Current MREFCs funding splits construction from operations  thus limiting support on ongoing work for  \gls{cyberinfrastructure},  there is little incentive in construction to build easy to operate systems.\footnote{This is also true for physical facilities e.g.  autonomous operation is usually not a requirement.}
If we blur the line between construction and operations for \gls{cyberinfrastructure} the issue becomes more one of long term support.


\nrec{Technology}{Technologist, Agency, Astronomer}{Short}{opspractices}{Improve long-term \gls{software} and service support}{Funding should  support repositories not just for code and data, but for computational environments. Use of proven standards in the wider research community for sharing and discovering runtime-ready \gls{software} using \gls{software} \gls{container} environments like \gls{Docker} and \gls{Docker}Hub but with domain specific curation
(e.g. BioContainers) is crutical\footnote{Critical and crucial \url{https://www.urbandictionary.com/define.php?term=crutical}} for both broader impacts of \gls{software} products and result
reproducibility as  compute environments continue to rapidly evolve with low emphasis given to
backward compatibility. }

Long term support could be improved by requiring proposals to state how code reuse and common practices will be used. Looking for  proposals which aim to push to the Code and
    \gls{API} communities (AstroGit? AstroContainers? AstroHub) and which aim to build on common
    \gls{software} development practices. Of course we should also foster development of those best practices
 based on best practices outside astronomy.
Concretely proposals could have  a line item for making \gls{software} reusable in funding budgets and funding agencies should see that as a good thing and try to develop metrics for success in the area.

We must also consider how to move to a more self service architecture in astronomy  such as GitOps \citep{Limoncelli:2018:GPM:3236386.3237207} - that requires some rigor but establishment of adhered to best practices would be a start.

Needless to say all of the code should be available under open licensing such as Apache (\gls{APL}) or Gnu (\gls{GPL}) public license.

\nrec{Technology}{Agency}{Medium}{cmdeploy}{Fund cross-mission deployment} {
    Missions that develop \gls{software} that can and should be adaptable to other common goals in other missions should be funded to develop and support cross-mission resources as part of this and other cyberinfrastuctures.
    }
Past examples
    of this success can be found as far back as the \gls{IRAF} environment and include now significantly
    more broadly adopted numpy, the cost of development and support have been paid back multifold
    across many funded projects and missions which did not have to develop their own versions
    of \gls{software}.

Deployability  is part of the problem but service oriented architectures are and will remain at the forefront for at least the next decade.
So we should now be thinking more of \gls{software} as a service and defining infrastructure as a service.
This would all funding agencies to push us more toward commodity compute and infrastructure services thus concentrating efforts on the astronomy problems at hand rather than the computer science problems.

%WOM - I do not understand  How does NSF drive us to Commodity as a service? Software is a product the same way data are and should be treated to the same community wide requirements.



Funding agencies could also  favor proposals that use/leverage existing \gls{software} solution, it may take time but this would be a positive fundamental change in astronomy \gls{software}.


%\NGaff{How do you build a sustaining model for software in this environment?  How do
%the priorities of multiple parties get addressed and prioritized? How do we make this more than the Data Plan's
%"all software will be available via open source license and posted to github"}

\subsection{Sustainability and effectiveness}
\label{sec:tech_sust}

An architecture as laid out in \secref{sec:refarc} gives us a framework to start a sustainable \gls{software} development in astronomy.
Software sustainability is a complex issue, with mixed results in astronomy --- see \secref{ssec:soft_sustain} for more on this complexity.
The approach laid out here, however, presents greater challenges than ever before in sustainability, as larger datasets and more complex infrastructure means that reinventing the wheel will become ever more costly.

By providing a reference architecture we can allow for more openness, collaboration, and when necessary, competition in each component.
While competition and alternatives can be useful in a controlled manner, i.e. funding two approaches for a specific component, by providing a reference architecture this can be adopted only when needed without interfering with other layers. We should also consider that this architecture may be good for a decade at which point it also should be revisited - such a refresh should be built in to our thinking from the start. This is critical for sustainability because sustainability is much more challenging if the architecture does not keep up with the technology, as more and more ``hacks'' become necessary until the house of cards comes toppling down.

The Astropy project has been successfully fostering a community approach to the user-facing end of Python astronomy. They do face challenges for funding and are beginning to tackle some management issue for an organically grown organisation. This has been successfully because they have worked hard to join the zeitgeist of open \gls{software} and have dedicated individuals who believe this is a useful project - and many users who agree. The project also produces useful tools.
The role of the Astropy project in the ecosystem can be misunderstood i.e. it is not meant to be a data management system or a replacement for a mission-specific toolchain, rather it is a toolbox that is accessible to astronomers for doing many of the tasks they want to use or understand. While the re-use and contribution to these tools by missions or observatories is desirable (see \secref{sec:software}), without a clear understanding of where the components lie in a larger architecture, it is almost impossible for astronomers and projects to understand how they can fit such components into their system. A reference architecture can thus help define where projects like this belong and how they fit with other efforts. For example, \gls{LSST} will not process data using \texttt{astropy} but will make their data products accessible and usable with particular Astropy project interfaces and tools. It has taken both projects a while to understand this delineation because  neither \gls{LSST} nor \texttt{AstroPy}  had a clear reference model to work with.

%How would you have LSST support PSP correction software that is used by others and get paid to do the support
%not just fit it in as they can.    There is arec for that above

% Frequently these large efforts are held together be a sort of benevolent dictator - Linux became hugely popular and the epitome of open software largely due to the efforts and decisions of Linus Torvalds. Everyone agreed what Linus said goes.
% Astronomy software is arguably a much more complex problem than Linux
% but perhaps if we can break it in to a set of  general areas we may find a leader in each area.
% There is no clear and good answer here and is definitely a good topic for some workshop sessions.

%How do you evolve this into a more general purpose system? Who is there to
%make the Linus (or Doug Tody in the early IRAF days) style decisions as opposed to having a FITS board? And how do we get general buy in to using
%this rather than simply hacking together a bad Perl script "that works for me" and putting it on github?  \emph{DO WE WANT
%THIS IN HERE AT ALL}


% This is covered in DM and refered to above (long term preservation) and in software and servics recs swmoney swecoplan
%\rec{fundci}{Funding of the CI - REDUNDANT WITH SOFTWARE BUT SHOULD BE SERVICE AFTER MISSIONS GO SO ITS ALSO DATA}{Projects should be funded to support the (was this the future preservation of data and services? The support for community based software development?)}






%\subsection{Infrastructure}\label{tiinfra}
%\begin{itemize}
%\item General/commodity vs. astronomy domain-specific - where can we pick up technology and apply it in new areas?
%\item Big Iron (supercomputing) ..  and or Containerization/virtualization
%\item Central data cloud .. (Code to data?)
%\item Cross facility, edge computing, reactive\footnote{\url{https://www.infoworld.com/article/3188924/software/a-brief-overview-of-reactive-systems.html}} computing
%\item Networks - e.g. what kind of infrastructure is missing?
%\item Commercial cloud computing services
%\item (adam) matching development and operations project-management frameworks to software and cyberinfrastructure (particularly where different than what is appropriate for big optomechanical infrastructure.)
%\end{itemize}










==> recs.tex <==
\section{Recommendations} \label{sec:recs}


%\Contributors{William O'Mullane <email@email>, }
%\bigskip


These tables summarize the recommendations in the document per audience we feel would be interested. Clicking the label or text will take you to the full recommendation in the document.\footnote{In a \gls{PDF} it may be useful to note that CMD $\leftarrow$ (CTRL on Windows/Linux) returns you to from whence you clicked.}
Please note that a recommendation may be aimed at multiple audiences and therefore may appear more than once in the tables below.
\input{audtabs.tex}

%\newpage

%\subsection{Three rec format}
%Least favorite way ..
%\input{tabs/tabs}
%\subsection{Single row format}
%\input{tabs/stabs}

%\subsection{Single row format per audience}

